The New Horizons Extended Mission Target: Arrokoth Search and Discovery

Following the Pluto fly-by of the New Horizons spacecraft, the mission provided a unique opportunity to explore the Kuiper Belt in-situ. The possibility existed to fly-by a Kuiper Belt object (KBO) as well as to observe additional objects at distances closer than are feasible from earth-orbit facilities. However, at the time of launch no KBOs were known about that were accessible by the spacecraft. In this paper we present the results of 10 years of observations and three uniquely dedicated efforts -- two ground-based using the Subaru Suprime Camera, the Magellan MegaCam and IMACS Cameras, and one with the Hubble Space Telescope -- to find such KBOs for study. In this paper we overview the search criteria and strategies employed in our work and detail the analysis efforts to locate and track faint objects in the galactic plane. We also present a summary of all of the KBOs that were discovered as part of our efforts and how spacecraft targetability was assessed, including a detailed description of our astrometric analysis which included development of an extensive secondary calibration network. Overall, these efforts resulted in the discovery of 89 KBOs including 11 which became objects for distant observation by New Horizons and (486958) Arrokoth which became the first post-Pluto fly-by destination.

==> 04obsFields.tex <==
\startlongtable
\begin{deluxetable}{ccccccc}
\tablecaption{2004 Search Fields\label{tbl-04obsFields}}
\tablewidth{0pt}
\tablehead{
\colhead{Field}&
\colhead{R.A.}&
\colhead{Dec.}&
}
\startdata
NH005&17:49:56.0&-23:03:45 \\
NH006&17:52:23.8&-23:03:45 \\
NH007&17:54:51.7&-23:03:45 \\
NH008&17:57:19.6&-23:03:45 \\
NH009&17:59:47.5&-23:03:45 \\
NH016&17:47:29.3&-22:36:45 \\
NH017&17:49:56.7&-22:36:45\\
NH018&17:52:24.1&-22:36:45 \\
NH019&17:54:51.5&-22:36:45 \\
NH020&17:57:18.9&-22:36:45 \\
NH021&17:59:46.3&-22:36:45 \\
NH022&18:02:13.6&-22:36:45 \\
NH025&17:40:09.7&-22:09:45 \\
NH026&17:42:36.7&-22:09:45\\
NH027&17:45:03.6&-22:09:45 \\
NH028&17:47:30.5&-22:09:45 \\
NH029&17:49:57.4&-22:09:45\\
NH030&17:52:24.3&-22:09:45\\
NH031&17:54:51.2&-22:09:45\\
NH032&17:57:18.1&-22:09:45\\
NH033&17:59:45.1&-22:09:45\\
NH034&18:02:12.0&-22:09:45 \\
NH035&18:04:38.9&-22:09:45 \\
NH036&18:07:05.8&-22:09:45\\
NH037&17:40:12.3&-21:42:45 \\
NH038&17:42:38.8&-21:42:45\\
NH039&17:45:05.2&-21:42:45 \\
NH040&17:47:31.7&-21:42:45\\
NH041&17:49:58.1&-21:42:45\\
NH042&17:52:24.5&-21:42:45\\
NH043&17:54:51.0&-21:42:45\\
NH044&17:57:17.4&-21:42:45\\
NH045&17:59:43.9&-21:42:45\\
NH046&18:02:10.3&-21:42:45 \\
NH047&18:04:36.8&-21:42:45 \\
NH048&18:07:03.2&-21:42:45\\
NH050&17:42:40.8&-21:15:45 \\
NH051&17:45:06.8&-21:15:45 \\
NH052&17:47:32.8&-21:15:45 \\
NH053&17:49:58.8&-21:15:45 \\
NH054&17:52:24.8&-21:15:45\\
NH055&17:54:50.8&-21:15:45\\
NH056&17:57:16.8&-21:15:45 \\
NH057&17:59:42.8&-21:15:45 \\
NH058&18:02:08.8&-21:15:45 \\
NH059&18:04:34.8&-21:15:45 \\
NH063&17:45:08.3&-20:48:45 \\
NH064&17:47:33.9&-20:48:45 \\
NH065&17:49:59.4&-20:48:45 \\
NH066&17:52:25.0&-20:48:45 \\
NH067&17:54:50.6&-20:48:45 \\
NH068&17:57:16.1&-20:48:45 \\
NH069&17:59:41.7&-20:48:45 \\
\enddata
\tablecomments{\scriptsize
The coordinates are all equinox J2000. }
\end{deluxetable}


==> Table_HSTobservations.tex <==
% This information comes from
% /net/wixer/raid/buie/nh/nhsearch/subaru/plan/nhfieldlist.txt
%
% select id& object& midtime& airmass& exptime& filtname from hinfo
%    where object like 'N%' and id like '%0';
% there are NH and NA fields

\begin{deluxetable}{cccccccccc}
\tablecaption{Summary of New Horizons Search Fields\label{tbl-hst-full}}
\tablewidth{0pt}
\tablehead{
\colhead{Dataset}&
\colhead{Target Name}&
\colhead{R.A.}&
\colhead{Dec.}&
\colhead{Starting Julian Date}&
\colhead{Calendar Date}&
\colhead{Exp. Duration}&
\colhead{Notes}\\
& & J2000& J2000& & & (hrs)& 
}
\startdata
01& KBO1-R6C3& 18:44:42.824& -20:55:52.32& 2456830.81797&  Jun-22-2014& 2.18& Guide Star Failure \\
02& KBO1-R6C3& 18:44:41.902& -20:55:53.28& 2456831.01196&  Jun-22-2014& 1.05& Guide Star Failure \\
03& KBO1-R6C4& 18:44:55.066& -20:55:53.02& 2456830.94559&  Jun-22-2014& 1.05& &\\
04& KBO1-R6C4& 18:44:54.435& -20:55:53.69& 2456831.07833&  Jun-22-2014& 1.05& &\\ 
05& KBO1-R7C3& 18:44:38.045& -20:53:36.62& 2456832.87027&  Jun-24-2014& 1.05& &\\
06& KBO1-R7C3& 18:44:37.410& -20:53:37.30& 2456833.00301&  Jun-24-2014& 1.05& &\\
07& KBO1-R7C4& 18:44:50.572& -20:53:37.01& 2456832.93664&  Jun-24-2014& 1.05& 2014MT69 \\
08& KBO1-R7C4& 18:44:49.937& -20:53:37.68& 2456833.06939&  Jun-24-2014& 1.05& 2014MT69 \\
09& KBO1-R7C5& 18:44:58.967& -20:53:41.77& 2456833.86583&  Jun-25-2014& 1.05& &\\
10& KBO1-R7C5& 18:44:58.330& -20:53:42.45& 2456833.99858&  Jun-25-2014& 1.05& &\\
11& KBO1-R7C6& 18:45:07.032& -20:53:46.86& 2456834.86137&  Jun-26-2014& 1.05& 2014MU69 \\
12& KBO1-R7C6& 18:45:06.393& -20:53:47.55& 2456834.99411&  Jun-26-2014& 1.05& 2014MU69 \\
13& KBO1-R7C7& 18:45:24.338& -20:53:41.91& 2456833.93221&  Jun-25-2014& 1.05& &\\
14& KBO1-R7C7& 18:45:23.701& -20:53:42.59& 2456834.06495&  Jun-25-2014& 1.05& &\\
15& KBO1-R7C8& 18:45:32.403& -20:53:46.88& 2456834.92775&  Jun-26-2014& 1.05& Guide Star Failure \\
16& KBO1-R7C8& 18:45:31.764& -20:53:47.58& 2456835.06049&  Jun-26-2014& 1.05& Guide Star Failure \\
17& KBO1-R8C2& 18:45:08.316& -20:50:31.25& 2456824.77483&  Jun-16-2014& 2.26& &\\
18& KBO1-R8C2& 18:45:07.691& -20:50:31.87& 2456824.91019&  Jun-16-2014& 2.05& &\\
19& KBO1-R8C3& 18:45:14.399& -20:50:38.08& 2456826.23308&  Jun-17-2014& 1.05& &\\
20& KBO1-R8C3& 18:45:13.782& -20:50:38.70& 2456826.36582&  Jun-17-2014& 1.05& &\\
21& KBO1-R8C4& 18:45:29.091& -20:50:36.25& 2456825.83485&  Jun-17-2014& 2.16& &\\
22& KBO1-R8C4& 18:45:27.858& -20:50:37.49& 2456826.10035&  Jun-17-2014& 1.05& &\\
23& KBO1-R8C5& 18:45:41.007& -20:50:37.14& 2456826.03397&  Jun-17-2014& 1.05& &\\
24& KBO1-R8C5& 18:45:40.390& -20:50:37.76& 2456826.16672&  Jun-17-2014& 1.05& &\\
25& KBO1-R8C6& 18:45:52.497& -20:50:38.41& 2456826.29947&  Jun-17-2014& 1.05& &\\
26& KBO1-R8C6& 18:45:51.934& -20:50:38.98& 2456826.44528&  Jun-17-2014& 2.28& &\\
27& KBO1-R8C7& 18:46:02.927& -20:50:40.69& 2456826.76582&  Jun-18-2014& 2.27& &\\
28& KBO1-R8C7& 18:46:02.049& -20:50:41.58& 2456827.02957&  Jun-18-2014& 1.05& &\\
29& KBO1-R9C2& 18:44:57.444& -20:48:21.21& 2456828.15789&  Jun-19-2014& 1.05& &\\
30& KBO1-R9C2& 18:44:56.938& -20:48:21.73& 2456828.29064&  Jun-19-2014& 1.05& &\\
31& KBO1-R9C3& 18:45:09.970& -20:48:21.59& 2456828.22427&  Jun-19-2014& 1.05& &\\
32& KBO1-R9C3& 18:45:09.463& -20:48:22.11& 2456828.35701&  Jun-19-2014& 1.05& &\\
33& KBO1-R9C4& 18:45:14.037& -20:48:30.66& 2456830.08274&  Jun-21-2014& 1.05& &\\
34& KBO1-R9C4& 18:45:13.526& -20:48:31.19& 2456830.21549&  Jun-21-2014& 1.05& &\\
35& KBO1-R9C5& 18:45:30.955& -20:48:26.37& 2456829.21988&  Jun-20-2014& 1.05& &\\
36& KBO1-R9C5& 18:45:30.446& -20:48:26.89& 2456829.35263&  Jun-20-2014& 1.05& &\\
37& KBO1-R9C6& 18:45:43.479& -20:48:26.57& 2456829.28626&  Jun-20-2014& 1.05& \\
38& KBO1-R9C6& 18:45:42.907& -20:48:27.16& 2456829.43245&  Jun-20-2014& 2.26& \\
39& KBO1-R9C7& 18:45:52.235& -20:48:30.63& 2456830.14913&  Jun-21-2014& 1.05& \\
40& KBO1-R9C7& 18:45:51.724& -20:48:31.17& 2456830.28187&  Jun-21-2014& 1.05& \\
41& KBO1-R0C7& 18:43:45.628& -21:10:15.65& 2456845.74450&  Jul-07-2014& 1.05& \\
42& KBO1-R0C7& 18:43:45.109& -21:10:16.26& 2456845.87722&  Jul-07-2014& 1.05& \\
43& KBO1-R0C8& 18:43:59.964& -21:10:16.03& 2456845.81088&  Jul-07-2014& 1.05& \\
44& KBO1-R0C8& 18:43:59.445& -21:10:16.64& 2456845.94360&  Jul-07-2014& 1.05& \\ 
45& KBO1-R0C9& 18:44:10.471& -21:10:20.86& 2456846.67358&  Jul-08-2014& 1.05& PT5 \\
46& KBO1-R0C9& 18:44:09.953& -21:10:21.48& 2456846.80631&  Jul-08-2014& 1.05& PT5 \\
47& KBO1-R1C6& 18:42:45.198& -21:09:10.66& 2456856.89648&  Jul-18-2014& 1.05& \\
48& KBO1-R1C6& 18:42:44.700& -21:09:11.30& 2456857.02929&  Jul-18-2014& 1.05& \\
49& KBO1-R1C7& 18:42:55.875& -21:09:15.84& 2456857.75979&  Jul-19-2014& 1.05& \\
50& KBO1-R1C7& 18:42:55.379& -21:09:16.48& 2456857.89262&  Jul-19-2014& 1.05& \\
51& KBO1-R1C8& 18:43:10.223& -21:09:16.19& 2456857.82622&  Jul-19-2014& 1.05& \\
52& KBO1-R1C8& 18:43:09.728& -21:09:16.83& 2456857.95904&  Jul-19-2014& 1.05& \\
53& KBO1-R1C9& 18:43:29.465& -21:09:10.14& 2456856.83013&  Jul-18-2014& 1.05& \\
54& KBO1-R1C9& 18:43:28.967& -21:09:10.79& 2456856.96294&  Jul-18-2014& 1.05& \\
55& KBO1-R2C5& 18:43:05.235& -21:06:25.74& 2456850.98749&  Jul-12-2014& 1.05& Moon \\
56& KBO1-R2C5& 18:43:04.724& -21:06:26.36& 2456851.12023&  Jul-12-2014& 1.05& Moon \\
57& KBO1-R2C6& 18:43:19.569& -21:06:26.20& 2456851.05388&  Jul-12-2014& 1.05& Moon \\
58& KBO1-R2C6& 18:43:19.051& -21:06:26.84& 2456851.18816&  Jul-12-2014& 1.05& Moon \\
59& KBO1-R2C7& 18:43:44.966& -21:06:13.10& 2456848.79723&  Jul-10-2014& 1.05& \\
60& KBO1-R2C7& 18:43:44.451& -21:06:13.73& 2456848.92998&  Jul-10-2014& 1.05& \\
61& KBO1-R2C8& 18:44:03.743& -21:06:08.06& 2456847.93449&  Jul-09-2014& 1.05& \\
62& KBO1-R2C8& 18:44:02.909& -21:06:09.06& 2456848.13359&  Jul-09-2014& 1.05& \\
63& KBO1-R2C9& 18:44:13.947& -21:06:13.26& 2456848.86362&  Jul-10-2014& 1.05& \\
64& KBO1-R2C9& 18:44:13.432& -21:06:13.88& 2456848.99637&  Jul-10-2014& 1.05& \\
65& KBO1-R3C5& 18:42:52.858& -21:04:39.97& 2456855.10360&  Jul-16-2014& 1.05& \\
66& KBO1-R3C5& 18:42:52.349& -21:04:40.61& 2456855.23759&  Jul-16-2014& 1.05& \\
67& KBO1-R3C6& 18:43:07.194& -21:04:40.41& 2456855.17001&  Jul-16-2014& 1.05& \\
68& KBO1-R3C6& 18:43:06.679& -21:04:41.06& 2456855.30558&  Jul-16-2014& 1.05& \\
69& KBO1-R3C7& 18:43:17.822& -21:04:45.49& 2456856.03412&  Jul-17-2014& 1.05& \\
70& KBO1-R3C7& 18:43:16.704& -21:04:46.92& 2456856.30023&  Jul-17-2014& 1.05& \\
71& KBO1-R3C8& 18:43:34.014& -21:04:43.41& 2456855.70125&  Jul-17-2014& 1.05& \\
72& KBO1-R3C8& 18:43:33.513& -21:04:44.05& 2456855.83406&  Jul-17-2014& 1.05& \\
73& KBO1-R3C9& 18:43:48.969& -21:04:42.82& 2456855.63486&  Jul-17-2014& 1.05& \\
74& KBO1-R3C9& 18:43:48.468& -21:04:43.46& 2456855.76767&  Jul-17-2014& 1.05& \\
75& KBO1-R4C4& 18:42:57.040& -21:02:15.02& 2456852.58067&  Jul-14-2014& 1.05& \\
76& KBO1-R4C4& 18:42:56.531& -21:02:15.65& 2456852.71344&  Jul-14-2014& 1.05& \\
77& KBO1-R4C5& 18:43:11.369& -21:02:15.49& 2456852.64707&  Jul-14-2014& 1.05& \\
78& KBO1-R4C5& 18:43:10.861& -21:02:16.12& 2456852.77984&  Jul-14-2014& 1.05& \\
79& KBO1-R4C6& 18:43:23.822& -21:02:18.23& 2456853.11179&  Jul-14-2014& 1.05& \\
80& KBO1-R4C6& 18:43:23.301& -21:02:18.88& 2456853.24766&  Jul-14-2014& 1.05& \\
81& KBO1-R4C7& 18:43:35.657& -21:02:21.68& 2456853.70932&  Jul-15-2014& 1.05& \\
82& KBO1-R4C7& 18:43:35.151& -21:02:22.31& 2456853.84211&  Jul-15-2014& 1.05& \\
83& KBO1-R4C8& 18:43:49.988& -21:02:21.92& 2456853.77573&  Jul-15-2014& 1.05& \\
84& KBO1-R4C8& 18:43:49.482& -21:02:22.55& 2456853.90851&  Jul-15-2014& 1.05& \\
85& KBO1-R5C4& 18:42:34.429& -21:00:42.84& 2456858.95512&  Jul-20-2014& 1.05& \\
86& KBO1-R5C4& 18:42:33.937& -21:00:43.49& 2456859.08793&  Jul-20-2014& 1.05& \\
87& KBO1-R5C5& 18:42:48.766& -21:00:43.29& 2456859.02154&  Jul-20-2014& 1.05& \\
88& KBO1-R5C5& 18:42:48.274& -21:00:43.93& 2456859.15435&  Jul-20-2014& 1.05& \\
89& KBO1-R5C6& 18:43:02.498& -21:00:44.45& 2456859.22076&  Jul-20-2014& 1.05& \\
90& KBO1-R5C6& 18:43:02.007& -21:00:45.10& 2456859.35358&  Jul-20-2014& 1.05& \\
91& KBO1-R5C7& 18:43:16.836& -21:00:44.74& 2456859.28719&  Jul-20-2014& 1.05& \\
92& KBO1-R5C7& 18:43:16.345& -21:00:45.39& 2456859.42000&  Jul-20-2014& 1.05& \\
93& KBO1-R5C8& 18:43:28.462& -21:00:48.52& 2456859.95096&  Jul-21-2014& 1.05& \\
94& KBO1-R5C8& 18:43:27.674& -21:00:49.57& 2456860.15016&  Jul-21-2014& 1.05& \\
95& KBO1-R6C5& 18:42:50.326& -20:58:40.41& 2456860.21653&  Jul-21-2014& 1.05& \\
96& KBO1-R6C5& 18:42:49.538& -20:58:41.46& 2456860.41573&  Jul-21-2014& 1.05& \\
97& KBO1-R6C6& 18:43:04.662& -20:58:40.74& 2456860.28294&  Jul-21-2014& 1.05& \\
98& KBO1-R6C6& 18:43:03.875& -20:58:41.78& 2456860.48214&  Jul-21-2014& 1.05& \\
99& KBO1-R6C7& 18:43:18.998& -20:58:41.00& 2456860.34935&  Jul-21-2014& 1.05& \\
A0& KBO1-R6C7& 18:43:18.212& -20:58:42.04& 2456860.54855&  Jul-22-2014& 1.05& \\
A1& KBO1-R6C8& 18:43:30.643& -20:58:44.75& 2456861.01336&  Jul-22-2014& 1.05& \\
A2& KBO1-R6C8& 18:43:29.860& -20:58:45.79& 2456861.21255&  Jul-22-2014& 1.05& \\
A3& KBO1-R10C2& 18:42:13.775& -20:48:10.60& 2456861.94279&  Jul-23-2014& 1.05& \\
A4& KBO1-R10C2& 18:42:12.998& -20:48:11.64& 2456862.14197&  Jul-23-2014& 1.05& \\
A5& KBO1-R10C3& 18:42:28.098& -20:48:11.07& 2456862.00920&  Jul-23-2014& 1.05& \\
A6& KBO1-R10C3& 18:42:27.321& -20:48:12.12& 2456862.20838&  Jul-23-2014& 1.05& \\
A7& KBO1-R10C4& 18:42:42.421& -20:48:11.48& 2456862.07560&  Jul-23-2014& 1.05& \\
A8& KBO1-R10C4& 18:42:41.645& -20:48:12.53& 2456862.27478&  Jul-23-2014& 1.05& \\
A9& KBO1-R10C5& 18:42:48.524& -20:48:22.96& 2456864.00081&  Jul-25-2014& 1.05& \\
B0& KBO1-R10C5& 18:42:48.051& -20:48:23.61& 2456864.13358&  Jul-25-2014& 1.05& \\
B1& KBO1-R10C6& 18:43:07.825& -20:48:16.44& 2456862.93869&  Jul-24-2014& 1.05& \\
B2& KBO1-R10C6& 18:43:07.054& -20:48:17.49& 2456863.13785&  Jul-24-2014& 1.05& \\
B3& KBO1-R10C7& 18:43:22.151& -20:48:16.62& 2456863.00509&  Jul-24-2014& 1.05& \\
B4& KBO1-R10C7& 18:43:21.380& -20:48:17.66& 2456863.20425&  Jul-24-2014& 1.05& \\
B5& KBO1-R11C2& 18:42:07.585& -20:46:18.55& 2456864.93007&  Jul-26-2014& 1.05& \\
B6& KBO1-R11C2& 18:42:06.827& -20:46:19.60& 2456865.12920&  Jul-26-2014& 1.05& \\
B7& KBO1-R11C3& 18:42:26.553& -20:46:12.63& 2456863.93441&  Jul-25-2014& 1.05& Guide Star Failure \\
B8& KBO1-R11C3& 18:42:26.080& -20:46:13.27& 2456864.06716&  Jul-25-2014& 1.05& Guide Star Failure \\
B9& KBO1-R11C4& 18:42:40.005& -20:46:14.19& 2456864.19994&  Jul-25-2014& 1.05& \\
C0& KBO1-R11C4& 18:42:39.768& -20:46:14.51& 2456864.26632&  Jul-25-2014& 1.05& \\
C1& KBO1-R11C5& 18:42:54.040& -20:46:14.88& 2456864.33271&  Jul-25-2014& 1.05& \\
C2& KBO1-R11C5& 18:42:53.858& -20:46:15.13& 2456864.39910&  Jul-25-2014& 1.05& \\
C3& KBO1-R11C6& 18:43:14.204& -20:46:07.13& 2456863.07147&  Jul-24-2014& 1.05& \\
C4& KBO1-R11C6& 18:43:13.434& -20:46:08.17& 2456863.27062&  Jul-24-2014& 1.05& \\
C5& KBO1-R12C1& 18:41:59.660& -20:44:08.88& 2456864.99644&  Jul-26-2014& 1.05& \\
C6& KBO1-R12C1& 18:41:58.904& -20:44:09.92& 2456865.19557&  Jul-26-2014& 1.05& \\
C7& KBO1-R12C2& 18:42:13.984& -20:44:09.37& 2456865.06282&  Jul-26-2014& 1.05& \\
C8& KBO1-R12C2& 18:42:13.228& -20:44:10.41& 2456865.26196&  Jul-26-2014& 1.05& \\
C9& KBO1-R12C3& 18:42:23.433& -20:44:16.54& 2456866.25755&  Jul-27-2014& 1.05& \\
D0& KBO1-R12C3& 18:42:22.970& -20:44:17.19& 2456866.39029&  Jul-27-2014& 1.05& \\
D1& KBO1-R12C4& 18:42:39.188& -20:44:14.89& 2456865.99208&  Jul-27-2014& 1.05& \\
D2& KBO1-R12C4& 18:42:38.724& -20:44:15.53& 2456866.12481&  Jul-27-2014& 1.05& \\
D3& KBO1-R12C5& 18:42:53.515& -20:44:15.14& 2456866.05846&  Jul-27-2014& 1.05& \\
D4& KBO1-R12C5& 18:42:53.051& -20:44:15.79& 2456866.19120&  Jul-27-2014& 1.05& \\
D5& KBO1-R13C1& 18:41:53.833& -20:42:16.82& 2456867.98311&  Jul-29-2014& 1.05& \\
D6& KBO1-R13C1& 18:41:53.378& -20:42:17.46& 2456868.11583&  Jul-29-2014& 1.05& \\
D7& KBO1-R13C2& 18:42:08.163& -20:42:17.27& 2456868.04948&  Jul-29-2014& 1.05& \\
D8& KBO1-R13C2& 18:42:07.708& -20:42:17.91& 2456868.18221&  Jul-29-2014& 1.05& \\
D9& KBO1-R13C3& 18:42:18.318& -20:42:23.59& 2456869.11131&  Jul-30-2014& 1.05& \\
E0& KBO1-R13C3& 18:42:17.592& -20:42:24.63& 2456869.31039&  Jul-30-2014& 1.05& \\
E1& KBO1-R13C4& 18:42:32.651& -20:42:23.89& 2456869.17767&  Jul-30-2014& 1.05& \\
E2& KBO1-R13C4& 18:42:31.926& -20:42:24.93& 2456869.37676&  Jul-30-2014& 1.05& \\
E3& KBO1-R13C5& 18:42:46.984& -20:42:24.11& 2456869.24405&  Jul-30-2014& 1.05& 2014OS393 \\
E4& KBO1-R13C5& 18:42:46.259& -20:42:25.15& 2456869.44314&  Jul-30-2014& 1.05& 2014OS393 \\
E5& KBO1-R14C1& 18:41:52.492& -20:40:18.74& 2456869.97398&  Jul-31-2014& 1.05& \\
E6& KBO1-R14C1& 18:41:52.047& -20:40:19.38& 2456870.10670&  Jul-31-2014& 1.05& \\
E7& KBO1-R14C2& 18:42:06.824& -20:40:19.16& 2456870.04035&  Jul-31-2014& 1.05& \\
E8& KBO1-R14C2& 18:42:06.379& -20:40:19.80& 2456870.17307&  Jul-31-2014& 1.05& \\
E9& KBO1-R14C3& 18:42:17.617& -20:40:24.63& 2456870.96939&  Aug-01-2014& 1.05& \\
F0& KBO1-R14C3& 18:42:17.178& -20:40:25.27& 2456871.10211&  Aug-01-2014& 1.05& \\
F1& KBO1-R14C4& 18:42:31.953& -20:40:24.89& 2456871.03575&  Aug-01-2014& 1.05& \\
F2& KBO1-R14C4& 18:42:31.462& -20:40:25.60& 2456871.16847&  Aug-01-2014& 1.05& \\
F3& KBO1-R15C1& 18:41:47.349& -20:38:26.51& 2456872.96010&  Aug-03-2014& 1.05& \\
F4& KBO1-R15C1& 18:41:46.921& -20:38:27.15& 2456873.09281&  Aug-03-2014& 1.05& \\
F5& KBO1-R15C2& 18:42:05.139& -20:38:21.76& 2456872.16382&  Aug-02-2014& 1.05& \\
F6& KBO1-R15C2& 18:42:04.706& -20:38:22.40& 2456872.29654&  Aug-02-2014& 1.05& \\
F7& KBO1-R15C3& 18:42:19.475& -20:38:22.05& 2456872.23019&  Aug-02-2014& 1.05& \\
F8& KBO1-R15C3& 18:42:19.042& -20:38:22.70& 2456872.36291&  Aug-02-2014& 1.05& \\
F9& KBO1-R15C4& 18:42:30.895& -20:38:26.60& 2456873.02648&  Aug-03-2014& 1.05& \\
G0& KBO1-R15C4& 18:42:30.467& -20:38:27.24& 2456873.15920&  Aug-03-2014& 1.05& \\
G1& KBO1-R16C1& 18:41:42.668& -20:36:34.13& 2456875.94640&  Aug-06-2014& 1.05& 2014PN70 \\
G2& KBO1-R16C1& 18:41:42.004& -20:36:35.16& 2456876.14547&  Aug-06-2014& 1.05& 2014PN70 \\
G3& KBO1-R16C2& 18:41:57.015& -20:36:34.46& 2456876.01277&  Aug-06-2014& 1.05& \\
G4& KBO1-R16C2& 18:41:56.352& -20:36:35.48& 2456876.21184&  Aug-06-2014& 1.05& \\
G5& KBO1-R16C3& 18:42:11.362& -20:36:34.71& 2456876.07913&  Aug-06-2014& 1.05& \\
G6& KBO1-R16C3& 18:42:10.700& -20:36:35.74& 2456876.27821&  Aug-06-2014& 1.05& \\
\enddata
\tablecomments{\scriptsize
}
\end{deluxetable}


==> tbl-11search.tex <==
% This started from Marc's file SummaryLogsOfObservingRuns_2011_2014.docx

\begin{deluxetable}{cccccccccc}
\tablecaption{Logs Notes from 2011-2014 Observing Runs\label{tbl-11search}}
\tablewidth{0pt}
\tablehead{
\colhead{Field}&
\colhead{UT Date}&
\colhead{UT Start Time}&
\colhead{FWHM ($''$)}&
\colhead{Quality}&
\colhead{Comments}&
}
\startdata
\
MA05&110428&04:56&0.7&1& 0.85${^\prime^\prime}$ at start, some elongation, transparency good\\
MA04&110428&05:40&0.6&1& Good image quality\\
MA07&110428&06:12&0.6&1& Up to 0.7`` for some exp.s\\
MA01&110428&06:48&0.55&1& Moonrise 06:57 UT\\
MA05&110428&07:26&0.5&1&  \\
MA04&110428&07:59&0.45&1& \\
MA07&110428&08:36&0.55&1& Cross meridian so more rotation\\
MA01&110428&09:19&0.55&1& \\
MA04&110428&09:51&0.55&3& Elevated bkg due to twilight\\
MA06&110429&04:52&1.0&1& 0.9-1.1${^\prime^\prime}$  Photometric all night\\
MA03&110429&05:29&0.8&1& $<$1.0${^\prime^\prime}$ down to 0.7${^\prime^\prime}$\\
MA02&110429&06:04&0.7&1& $<$0.7${^\prime^\prime}$\\
MA00&110429&06:36&1.1&1& 1.0-1.2${^\prime^\prime}$\\
MA08&110429&07:14&0.8&1& \\
MA03&110429&07:54&0.65&1& \\
MA06&110429&08:31&0.65&1&  only 11 exp.s taken\\
MA02&110429&09:01&0.6&1& \\
MA00&110429&09:33&0.75&1& \\
MA08&110430&04:47&0.90&1&  1${^\prime^\prime}$-0.8${^\prime^\prime}$\\
MA05&110430&05:17&0.80&2& nixed, focus let go on 6th image\\
MA05&110430&05:40&0.80&1&  \\
MA07&110430&06:15&0.75&1& \\
MA01&110430&06:55&0.70&1& \\
MA04&110430&07:27&0.65&1& \\
MA08&110430&07:59&0.60&1& last couple at 0.9\\
MA05&110430&08:36&0.90&1&  first 3 frames 1.1${^\prime^\prime}$- 0.9${^\prime^\prime}$,$+$12 more $<$0.8${^\prime^\prime}$\\
MA07&110430&09:15&0.65&1&  0.7${^\prime^\prime}$-0.6${^\prime^\prime}$ \\
MA04&110430&09:49&0.65&3&   $\sim$only 5 frames \\
MA06&110501&04:49&1.0&1& Clear Skies, photometric conditions throughout\\
MA03&110501&05:25&0.9&1& \\
MA02&110501&05:58&1.0&1& \\
MA00&110501&06:34&0.9&1&  0.8-1.0${^\prime^\prime}$\\
MA04&110501&07:20&0.7&1& \\
MA06&110501&08:01&0.65&1& \\
MA03&110501&08:45&0.65&1& 0.6-0.7${^\prime^\prime}$  pointing difference $$<$$ 1${^\prime^\prime}$\\
MA00&110501&09:34&0.75&2& 0.7-0.8${^\prime^\prime}$  incomplete set - only 9x120s \\
MA04&110502&06:30&0.60&1& Photometric throughout\\
MA04&110502&07:00&0.50&1& \\
MA04&110502&07:30&0.50&1& \\
MA04&110502&08:00&0.45&1& \\
MA04&110503&06:34&0.40&1& Photometric throughout\\
MA04&110503&07:15&0.40&1& \\
MA04&110503&07:50&0.40&1& \\
MA04&110503&08:25&0.40&1& \\
MA03&110503&09:11&0.38&1& \\
MA03&110503&09:40&0.42&2& Probable significant twilight \\
MA01&110504&08:19&0.50&1& Photometric. 0.45-0.55${^\prime^\prime}$, some images 0.6${^\prime^\prime}$\\
MA01&110504&08:50&0.50&1& \\
MA01&110504&09:20&0.50&1& \\
MA01&110504&09:50&0.50&3& $+$6 exp.s, probable significant twilight \\
MA05&110505&08:36&0.80&1& Photometric, variable seeing.   0.55-0.8${^\prime^\prime}$ \\
MA05&110505&09:10&0.70&1& Photometric, variable seeing.     0.55-0.8${^\prime^\prime}$   \\
MA05&110505&09:40&0.60&2& Photometric, variable seeing. 4 frames elevated b/g, 0.55-0.8${^\prime^\prime}$\\
MA07&110506&08:41&0.75&3& Variable clouds, only 6 clean frames.  Last 09:00  \\
MB04&110527&05:56&0.9&2&  1${^\prime^\prime}$ - 0.8${^\prime^\prime}$ elongation in a couple images (wind?)\\
MB01&110527&06:38&0.9&2&  1${^\prime^\prime}$ - 0.8${^\prime^\prime}$\\
MB04&110527&07:10&0.9&2&  0.9${^\prime^\prime}$ - 0.7${^\prime^\prime}$ - 1.1${^\prime^\prime}$\\
MB01&110527&07:42&1.1&2&  1${^\prime^\prime}$ - 1.2${^\prime^\prime}$ - 1.0${^\prime^\prime}$\\
MB04&110527&08:22&1.2&3&  1.1${^\prime^\prime}$ - 1.5${^\prime^\prime}$ - 1.0${^\prime^\prime}$ seeing too poor, not likely acceptable \\
MB01&110527&09:01&1.1&2&  1.1${^\prime^\prime}$ - 1.2${^\prime^\prime}$ - 1.0${^\prime^\prime}$ \\
MB04&110527&09:34&1.3&3&  1.2${^\prime^\prime}$ - 1.5${^\prime^\prime}$ - 1.1${^\prime^\prime}$ \\
MB04&110531&04:40&0.75&2&  0.8-0.7 \\
MB01&110531&05:13&0.7&1& \\
MB03&110531&05:43&0.6&1& \\
MB04&110531&06:19&0.6&1& \\
MB01&110531&06:56&0.6&1& last frame lost due to field rotation error\\
MB03&110531&07:29&0.55&1& \\
MB04&110531&08:01&0.6&1& \\
MB01&110531&08:42&0.7&1& \\
MB03&110531&09:16&0.7&1& \\
MB05&110531&09:51&0.9&2& \\
MB04&110604&02:15&0.9&1&  0.8${^\prime^\prime}$-1.0${^\prime^\prime}$ \\
MB05&110604&02:56&0.85&1&  0.8${^\prime^\prime}$-0.9${^\prime^\prime}$ \\
MB07&110604&03:28&0.9&3&  0.9${^\prime^\prime}$ only one exp. then closed to wind\\
MB07&110604&06:50&0.9&1&  0.8${^\prime^\prime}$-1.0${^\prime^\prime}$ seeing flared in one exp. to 1.3${^\prime^\prime}$\\
MB05&110604&07:23&1.3&1&  0.9${^\prime^\prime}$-1.5${^\prime^\prime}$ seeing jumping around but mostly above 1.2${^\prime^\prime}$\\
MB05&110604&07:57&1.15&1&  1.0${^\prime^\prime}$-1.3${^\prime^\prime}$ seeing continued to vary\\
MB05&110604&08:29&1.0&1&  0.9${^\prime^\prime}$-1.1${^\prime^\prime}$ \\
MB07&110604&09:05&1.1&1&  0.9${^\prime^\prime}$-1.2${^\prime^\prime}$ seeing flared up to 1.4${^\prime^\prime}$ in 2 exp., took extra exp.\\
MB05&110604&09:42&1.2&1&  1.0${^\prime^\prime}$-1.4${^\prime^\prime}$ \\
MB05&110604&10:14&1.3&2&  1.2${^\prime^\prime}$-1.4${^\prime^\prime}$ only 7 exp.s in the set\\
MC04&110701&02:08&0.7&1&  0.65-0.75${^\prime^\prime}$\\
MC01&110701&02:39&0.65&1&  0.6-0.7${^\prime^\prime}$\\
MC03&110701&03:10&0.6&1&  0.5-0.7${^\prime^\prime}$\\
MC05&110701&03:41&0.55&1&  0.5-0.6${^\prime^\prime}$\\
MC04&110701&04:12&0.7&1&  0.55-0.8${^\prime^\prime}$\\
MC01&110701&04:42&0.8&1&  0.7-0.9${^\prime^\prime}$ \\
MC03&110701&05:13&0.8&1&  0.7-0.9${^\prime^\prime}$ \\
MC05&110701&05:44&0.8&1&  0.7-0.9${^\prime^\prime}$ \\
MC04&110701&06:14&0.8&1&  0.7-0.9${^\prime^\prime}$\\
MC01&110701&06:45&0.8&1&  0.7-0.9${^\prime^\prime}$\\
MC03&110701&07:16&0.8&1&  0.7-0.9${^\prime^\prime}$ \\
MC05&110701&07:47&0.9&1&  0.75-1.1${^\prime^\prime}$\\
MC07&110701&08:17&1.0&1&  0.8-1.2${^\prime^\prime}$  a couple of extra exp.s in this set\\
MC00&110702&00:12&0.80&1&  0.75-0.85\\
MC07&110702&00:43&0.75&1&  0.65-0.85${^\prime^\prime}$\\
MC02&110702&01:14&0.75&1&  0.65-0.9${^\prime^\prime}$\\
MC06&110702&01:44&0.75&1&  0.65-0.9${^\prime^\prime}$\\
MC08&110702&02:17&0.85&1&  0.65-1.1${^\prime^\prime}$\\
MC00&110702&02:47&0.70&1&  0.6-0.75${^\prime^\prime}$\\
MC07&110702&03:18&0.70&1&  0.65-0.75${^\prime^\prime}$\\
MC02&110702&03:48&0.65&1&  0.55-0.75${^\prime^\prime}$ \\
MC06&110702&04:19&0.80&1&  0.7-0.85${^\prime^\prime}$  2 frames at 1-1.1${^\prime^\prime}$ meridian crossing, extra frames \\
MC08&110702&04:55&0.90&1&  0.8-1.0${^\prime^\prime}$\\
MC00&110702&05:26&0.75&1&  0.65-0.8${^\prime^\prime}$\\
MC07&110702&05:57&0.75&1&  0.7-0.8${^\prime^\prime}$\\
MC02&110702&06:27&0.80&1&  0.75-0.85${^\prime^\prime}$  readout glitch in one frame, added replacement\\
MC06&110702&07:00&0.85&1&  0.75-0.95${^\prime^\prime}$  readout glitch in one frame, added replacement\\
MC08&110702&07:34&1.05&1&  0.95-1.1${^\prime^\prime}$\\
MC04&110702&08:05&1.20&1&  1.0-1.4${^\prime^\prime}$ a few extra frames ?utility\\
MD06&110722&23:34&0.7&1&  0.6-0.8 variable (poor in CCD01,CCD06 coma and astig), steady with time\\
MD07&110723&00:04&0.7&1&  0.6-0.8  \\
MD08&110723&00:36&0.7&1&  0.6-0.8  \\
MD06&110723&01:07&0.7&1&  0.6-0.8  \\
MD07&110723&01:37&0.55&1&  0.5-0.6 for 75\% array with poor IQ on most of CCD01 and CCD06 \\
MD06&110723&02:27&0.65&1&  0.6-0.7 focus offset applied before exp. earthquake during last exp.!\\
MD07&110723&03:02&0.65&1&  0.5-0.8\\
MD08&110723&23:15&0.8&1&   0.6-1.0 variable seeing\\
MD00&110723&23:59&0.8&1&   0.7-0.9\\
MD06&110724&00:30&0.7&1&   0.6-0.8\\
MD08&110724&01:01&0.7&1&   0.6-0.8\\
MD00&110724&01:32&0.65&1&   0.6-0.7\\
MD07&110724&02:03&0.65&1&   0.6-0.7 some wind shake \\
MD08&110724&02:34&0.65&1&   0.6-0.8 elevated winds \\
MD00&110724&03:05&0.6&1&   0.5-0.7\\
MD01&110730&23:29&0.8&1&   0.74-0.88${^\prime^\prime}$\\
MD01&110731&00:01&0.85&3&   0.66-1.0${^\prime^\prime}$  Possible cloud?\\
MD04&110731&00:32&0.65&3&   0.6-0.7${^\prime^\prime}$  Possible cloud?\\
MD02&110731&01:03&0.8&3&   0.8${^\prime^\prime}$ lost guide star/cloud on image 8 (of 11); Closed telescope, clouds\\
MD02&110731&06:01&1.0&3&   0.9-1.1${^\prime^\prime}$  Probably some cloud\\
MD01&110731&06:34&1.1&3&   1.1${^\prime^\prime}$ Probably some cloud \\
ME01&110827&23:36&1.1&1&  11x100s\\
ME02&110828&00:13&1.4&2&  6x100s  shutdown due to high winds at end of exp.\\
ME01&110828&02:20&1.2&1&  11x100s\\
ME02&110828&03:51&1.1&1&   11x100s \\
ME07&110828&03:21&1.2&1&   11x100s \\
ME01&110828&03:54&1.3&1&   11x100s \\
ME02&110828&04:25&1.6&1&   11x100s  wind speed high\\
ME02&110828&23:13&1.0&2& 0.9${^\prime^\prime}$ - 1.1${^\prime^\prime}$  acquired in 12-18 degree twilight\\
ME07&110828&23:45&1.2&1& 1.1${^\prime^\prime}$ - 1.3${^\prime^\prime}$ \\
ME06&110829&00:17&0.95&1& 0.8 - 1.1${^\prime^\prime}$\\
ME08&110829&00:47&0.75&1& 0.7${^\prime^\prime}$ - 0.8${^\prime^\prime}$\\
ME07&110829&01:18&0.95&1& 0.7${^\prime^\prime}$ - 1.2${^\prime^\prime}$\\
ME06&110829&01:50&1.25&1& 1.1${^\prime^\prime}$ - 1.4${^\prime^\prime}$\\
ME08&110829&02:20&1.30&1& 1.0${^\prime^\prime}$ - 1.6${^\prime^\prime}$\\
ME07&110829&02:52&1.15&1& 1.0${^\prime^\prime}$ - 1.3${^\prime^\prime}$\\
ME06&110829&03:24&1.40&1& 1.2${^\prime^\prime}$ - 1.6${^\prime^\prime}$\\
ME08&110829&03:55&1.50&1& 1.2${^\prime^\prime}$ - 1.8${^\prime^\prime}$\\
ME01&110829&23:14&1.15&1& airmass 1.06-1.03,  1.0${^\prime^\prime}$ - 1.3${^\prime^\prime}$  acquired after 12 deg twilight\\
ME10&110829&23:44&1.20&1& airmass 1.03-1.02,  1.1${^\prime^\prime}$ - 1.3${^\prime^\prime}$\\
ME04&110830&00:15&1.30&1& airmass 1.01-1.01,  1.3${^\prime^\prime}$\\
ME06&110830&00:46&1.70&1& airmass 1.01-1.02,  1.4${^\prime^\prime}$ - 2.0${^\prime^\prime}$\\
ME10&110830&01:16&1.50&1& airmass 1.02-1.05,  1.5${^\prime^\prime}$\\
ME04&110830&01:48&1.20&1& airmass 1.05-1.09,  1.2${^\prime^\prime}$\\
ME06&110830&02:19&1.65&1& airmass 1.10-1.17,  1.3${^\prime^\prime}$ - 2.0${^\prime^\prime}$\\
ME10&110830&02:50&1.75&1& airmass 1.17-1.26,  1.5  - 2.0${^\prime^\prime}$\\
ME04&110830&03:21&2.10&1& airmass 1.27-1.71,  1.2${^\prime^\prime}$ - 3.0${^\prime^\prime}$ on ME04 for the remainder of night\\
MF10&120417&06:47&0.65&1&\\
MF01&120417&07:38&0.5&1&\\
MF01&120417&08:09&0.7&1& 0.6-0.8${^\prime^\prime}$  one frame at 0.9${^\prime^\prime}$, something came thru\\
MF01&120417&08:35&0.55&1& 0.5-0.6${^\prime^\prime}$\\
MF01&120417&09:06&0.52&1& 0.5-0.55${^\prime^\prime}$\\
MF01&120417&09:31&0.55&1& 0.5-0.6${^\prime^\prime}$\\
MF01&120417&09:57&0.55&2& 0.5-0.6${^\prime^\prime}$  set of only 5 exp.s\\
MF10&120418&05:20&0.90&1& 0.8-1.0${^\prime^\prime}$ Thin cirrus, $<$10\% extinction (keep quality class at 1)\\
MF01&120418&05:56&0.62&1& 0.55-0.7${^\prime^\prime}$\\
MF01&120418&06:27&0.70&1& 0.6-0.8${^\prime^\prime}$\\
MF01&120418&07:01&0.5&1& \\
MF01&120418&07:37&0.55&1& 0.5-0.6${^\prime^\prime}$\\
MF01&120418&08:08&0.60&1& 0.55-0.65${^\prime^\prime}$\\
MF01&120418&08:42&0.57&1& $<$0.5-0.65${^\prime^\prime}$\\
MF01&120418&09:13&0.57&1& 0.55-0.6${^\prime^\prime}$\\
MF01&120418&09:44&0.55&2& 0.5-0.6  sky bkg coming up after first 5 exp.\\
MF10&120419&05:15&0.90&1& 0.8-1.0${^\prime^\prime}$\\
MF10&120419&05:50&0.85&1& 0.8-0.9${^\prime^\prime}$\\
MF10&120419&06:25&0.72&1& 0.65-0.8${^\prime^\prime}$\\
MF01&120419&07:03&0.62&1&  0.6-0.65${^\prime^\prime}$\\
MF01&120419&07:37&0.60&1& 0.55-0.65${^\prime^\prime}$\\
MF01&120419&08:08&0.62&1& 0.55-0.7${^\prime^\prime}$\\
MF01&120419&08:38&0.57&1& 0.55-0.6${^\prime^\prime}$\\
MF01&120419&09:13&0.62&1& 0.55-0.7${^\prime^\prime}$\\
MF01&120419&09:43&0.60&1& 0.55-0.65${^\prime^\prime}$ only 10 in this set\\
MF10&120420&05:13&1.10&1&  1.0-1.2${^\prime^\prime}$  one at 1.6${^\prime^\prime}$ 12x120s r \\
MF10&120420&05:45&0.95&4&  0.9-1.0${^\prime^\prime}$  astrometric dither 3x30s r\\
MF01&120420&05:53&0.90&1&  0.8-1.0${^\prime^\prime}$  12x120s r\\
MF01&120420&06:24&0.90&4&  0.9${^\prime^\prime}$      astrometric dither 3x30s r\\
MF01&120420&06:28&0.85&1&  0.8-0.9${^\prime^\prime}$  12x120s r\\
MF04&120420&07:03&0.77&4&  0.75-0.8${^\prime^\prime}$  astrometric dither 3x30s r\\
MF04&120420&07:10&0.72&1&  0.65-0.8${^\prime^\prime}$  12x120s r\\
MF04&120420&07:44&0.67&1&  0.6-0.75${^\prime^\prime}$  12x120s r\\
MF04&120420&08:15&0.77&1&  0.7-0.85${^\prime^\prime}$  9x120s r\\
MF04&120420&08:41&0.85&1&  0.8-0.9${^\prime^\prime}$   9x120s r astigmatic ... adjusted collimation and WFS\\
MF04&120420&09:23&0.70&1&  0.65-0.75${^\prime^\prime}$ 12x120s r\\
MF04&120420&09:55&0.82&2&  0.65-1.0${^\prime^\prime}$  8x120s r bkg coming up on last frames\\
MF04&120420&10:16&0.60&4&  0.6${^\prime^\prime}$       120s i for comparison\\
MF04&120421&05:27&1.30&1&   1.1-1.6${^\prime^\prime}$  12x120s r.  Clear and photometric throughout\\
MF04a&120421&06:03&1.20&4&   1.1-1.3${^\prime^\prime}$  astrometric dither 5x30s r\\
MF10a&120421&06:14&1.50&4&   1.4-1.6${^\prime^\prime}$  astrometric dither 5x30s r\\
MF10a&120421&06:24&1.37&4&   1.25-1.5${^\prime^\prime}$ astrometric dither 5x30s r\\
MF01a&120421&06:34&1.42&4&   1.25-1.6${^\prime^\prime}$ astrometric dither 5x30s r\\
MF01a&120421&06:44&1.10&4&   1.0-1.2${^\prime^\prime}$  astrometric dither 5x30s r\\
MF04a&120421&06:59&1.15&4&   1.1-1.2${^\prime^\prime}$  astrometric dither 5x30s r\\
MF04&120421&07:16&0.95&1&   0.8-1.1${^\prime^\prime}$  12x120s r\\
MF04&120421&07:47&0.80&4&   0.8${^\prime^\prime}$      120s i \\
MF04&120421&08:06&0.90&1&   0.8-1.0${^\prime^\prime}$  12x120s r\\
MF04&120421&08:39&0.77&1&   0.75-0.8${^\prime^\prime}$ 12x120s r\\
MF04&120421&09:16&0.90&1&   0.8-1.0${^\prime^\prime}$  12x120s r\\
MF04&120421&09:47&0.92&2&   0.85-1.0${^\prime^\prime}$  8x120s r\\
MF04&120422&05:15&1.40&1&  1.2-1.6${^\prime^\prime}$  12x120s r (just because I could)\\
XX13&120422&05:56&1.20&1&  1.2${^\prime^\prime}$      3x120s r (look ahead 2013)\\
XX13o&120422&06:09&1.30&1&  1.3${^\prime^\prime}$      3x120s r (offset 400${^\prime^\prime}$S from nominal center for bright star)\\
XX14&120422&06:34&1.30&1&  1.3${^\prime^\prime}$      3x120s r (look ahead 2014)\\
XX15&120422&06:51&1.30&1&  1.3${^\prime^\prime}$      3x120s r (look ahead 2015)\\
MF04&120422&07:04&1.20&1&  1.1-1.3${^\prime^\prime}$  12x120s r (we do not really need more at this image quality)\\
MG07&120524&05:00&0.65&1&  0.6-0.7${^\prime^\prime}$\\
MG07&120524&05:30&0.65&1&  0.6-0.7${^\prime^\prime}$\\
MG07&120524&06:00&0.65&1&  0.6-0.7${^\prime^\prime}$\\
MG07&120524&06:30&0.65&1&  0.6-0.7${^\prime^\prime}$\\
MG07&120524&07:00&0.65&1&  0.6-0.7${^\prime^\prime}$\\
MG03&120524&07:22&0.90&1&  0.8-1.0${^\prime^\prime}$  Stayed on field till 08:08, then closed due to winds\\
MH07&120615&03:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120615&04:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120615&05:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120615&06:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120615&07:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120616&03:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120616&04:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120616&05:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120616&06:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MH07&120616&07:00&0.80&1&  Windy.  Approx log reconstructed from sparse notes\\
MI00	& 2012-07-16 & 23:10:27 & 1.67 & 1 & iff0058c1.fits high airmass, meant for astrometry\\
MI01 & 2012-07-16 & 23:12:38 & 1.56 & 1 & iff0059c1.fits\\
MI02 & 2012-07-16 & 23:14:46 & 1.82 & 1 & iff0060c1.fits\\
MI03 & 2012-07-16 & 23:16:43 & 1.85 & 1 & iff0061c1.fits\\
MI04 & 2012-07-16 & 23:18:54 & 1.89 & 1 & iff0062c1.fits\\
MI05 & 2012-07-16 & 23:20:58 & 1.93 & 1 & iff0063c1.fits\\
MI06 & 2012-07-16 & 23:23:03 & 1.98 & 1 & iff0064c1.fits\\
MI07 & 2012-07-16 & 23:25:10 & 2.29 & 1 & iff0065c1.fits\\
MI08 & 2012-07-16 & 23:27:17 & 2.19 & 1 & iff0066c1.fits\\
MI05 & 2012-07-16 & 23:33:18 & 1.48 & 1 & iff0067c1.fits airmass ~1.8\\
MI05 & 2012-07-16 & 23:39:42 & 1.40 & 1 & iff0068c1.fits\\
MI05 & 2012-07-16 & 23:46:05 & 1.58 & 1 & iff0069c1.fits\\
MI05 & 2012-07-16 & 23:52:28 & 1.29 & 1 & iff0070c1.fits\\
MI05 & 2012-07-16 & 23:58:52 & 1.38 & 1 & iff0071c1.fits\\
MI05 & 2012-07-17 & 00:05:16 & 1.34 & 1 & iff0072c1.fits\\
MI05 & 2012-07-17 & 00:11:39 & 1.28 & 1 & iff0073c1.fits\\
MI05 & 2012-07-17 & 00:18:02 & 1.07 & 1 & iff0074c1.fits\\
MI05 & 2012-07-17 & 00:24:25 & 1.12 & 1 & iff0075c1.fits\\
MI05 & 2012-07-17 & 00:30:48 & 1.32 & 1 & iff0076c1.fits\\
MI05 & 2012-07-17 & 00:37:12 & 1.52 & 1 & iff0077c1.fits\\
MI05 & 2012-07-17 & 00:43:35 & 1.46 & 1 & iff0078c1.fits\\
MI05 & 2012-07-17 & 00:49:58 & 1.26 & 1 & iff0079c1.fits\\
MI05 & 2012-07-17 & 00:56:21 & 1.20 & 1 & iff0080c1.fits\\
MI05 & 2012-07-17 & 01:02:45 & 1.18 & 1 & iff0081c1.fits\\
MI05 & 2012-07-17 & 01:09:09 & 1.37 & 1 & iff0082c1.fits\\
MI05 & 2012-07-17 & 01:15:32 & 1.72 & 1 & iff0083c1.fits\\
MI05 & 2012-07-17 & 01:21:56 & 1.42 & 1 & iff0084c1.fits\\
MI05 & 2012-07-17 & 01:28:19 & 1.10 & 1 & iff0085c1.fits\\
MI05 & 2012-07-17 & 01:34:42 & 1.00 & 1 & iff0086c1.fits\\
MI03 & 2012-07-17 & 01:42:20 & 0.98 & 1 & iff0087c1.fits\\
MI03 & 2012-07-17 & 01:48:44 & 1.09 & 1 & iff0088c1.fits\\
MI03 & 2012-07-17 & 01:55:07 & 1.01 & 1 & iff0089c1.fits\\
MI03 & 2012-07-17 & 02:01:30 & 1.18 & 1 & iff0090c1.fits\\
MI03 & 2012-07-17 & 02:07:53 & 0.99 & 1 & iff0091c1.fits\\
MI03 & 2012-07-17 & 02:14:16 & 1.04 & 1 & iff0092c1.fits\\
MI03 & 2012-07-17 & 02:20:40 & 0.98 & 1 & iff0093c1.fits\\
MI03 & 2012-07-17 & 02:27:04 & 1.13 & 1 & iff0094c1.fits\\
MI03 & 2012-07-17 & 02:33:27 & 1.41 & 1 & iff0095c1.fits\\
MI03 & 2012-07-17 & 02:39:51 & 1.23 & 1 & iff0096c1.fits\\
MI03 & 2012-07-17 & 02:46:15 & 1.30 & 1 & iff0097c1.fits\\
MI03 & 2012-07-17 & 02:52:38 & 1.16 & 1 & iff0098c1.fits\\
MI03 & 2012-07-17 & 02:59:01 & 1.11 & 1 & iff0099c1.fits\\
MI03 & 2012-07-17 & 03:05:25 & 1.09 & 1 & iff0100c1.fits\\
MI03 & 2012-07-17 & 03:11:48 & 1.01 & 1 & iff0101c1.fits\\
MI03 & 2012-07-17 & 03:18:11 & 0.97 & 1 & iff0102c1.fits\\
MI03 & 2012-07-17 & 03:24:34 & 0.93 & 1 & iff0103c1.fits\\
MI03 & 2012-07-17 & 03:30:58 & 0.96 & 1 & iff0104c1.fits\\
MI03 & 2012-07-17 & 03:37:21 & 0.96 & 1 & iff0105c1.fits\\
MI03 & 2012-07-17 & 03:43:44 & 0.90 & 1 & iff0106c1.fits\\
MI01 & 2012-07-17 & 03:50:21 & 0.90 & 1 & iff0107c1.fits\\
MI01 & 2012-07-17 & 03:56:44 & 0.94 & 1 & iff0108c1.fits\\
MI01 & 2012-07-17 & 04:03:07 & 0.95 & 1 & iff0109c1.fits\\
MI01 & 2012-07-17 & 04:09:30 & 0.86 & 1 & iff0110c1.fits\\
MI01 & 2012-07-17 & 04:15:53 & 0.81 & 1 & iff0111c1.fits\\
MI01 & 2012-07-17 & 04:22:17 & 0.79 & 1 & iff0112c1.fits\\
MI01 & 2012-07-17 & 04:28:40 & 0.78 & 1 & iff0113c1.fits\\
MI01 & 2012-07-17 & 04:35:04 & 0.89 & 1 & iff0114c1.fits\\
MI01 & 2012-07-17 & 04:41:28 & 0.87 & 1 & iff0115c1.fits\\
MI01 & 2012-07-17 & 04:47:51 & 0.88 & 1 & iff0116c1.fits\\
MI01 & 2012-07-17 & 04:54:14 & 0.92 & 1 & iff0117c1.fits\\
MI01 & 2012-07-17 & 05:00:38 & 1.00 & 1 & iff0118c1.fits\\
MI01 & 2012-07-17 & 05:07:01 & 1.27 & 1 & iff0119c1.fits\\
MI01 & 2012-07-17 & 05:13:24 & 0.85 & 1 & iff0120c1.fits\\
MI01 & 2012-07-17 & 05:19:47 & 0.84 & 1 & iff0121c1.fits\\
MI01 & 2012-07-17 & 05:26:10 & 0.76 & 1 & iff0122c1.fits\\
MI01 & 2012-07-17 & 05:32:34 & 0.84 & 1 & iff0123c1.fits\\
MI01 & 2012-07-17 & 05:38:57 & 0.86 & 1 & iff0124c1.fits\\
MI01 & 2012-07-17 & 05:45:20 & 0.86 & 1 & iff0125c1.fits\\
MI01 & 2012-07-17 & 05:51:43 & 0.88 & 1 & iff0126c1.fits\\
MI04 & 2012-07-17 & 05:58:15 & 0.82 & 1 & iff0127c1.fits\\
MI04 & 2012-07-17 & 06:04:38 & 0.85 & 1 & iff0128c1.fits\\
MI04 & 2012-07-17 & 06:11:01 & 0.83 & 1 & iff0129c1.fits\\
MI04 & 2012-07-17 & 06:17:24 & 0.87 & 1 & iff0130c1.fits\\
MI04 & 2012-07-17 & 06:23:47 & 0.95 & 1 & iff0131c1.fits\\
MI04 & 2012-07-17 & 06:30:11 & 1.16 & 1 & iff0132c1.fits\\
MI04 & 2012-07-17 & 06:36:34 & 1.20 & 1 & iff0133c1.fits\\
MI04 & 2012-07-17 & 06:42:57 & 1.04 & 1 & iff0134c1.fits\\
MI04 & 2012-07-17 & 06:49:21 & 1.23 & 1 & iff0135c1.fits\\
MI04 & 2012-07-17 & 06:55:44 & 1.05 & 1 & iff0136c1.fits\\
MI04 & 2012-07-17 & 07:02:07 & 1.03 & 1 & iff0137c1.fits\\
MI04 & 2012-07-17 & 07:08:31 & 0.90 & 1 & iff0138c1.fits\\
MI04 & 2012-07-17 & 07:14:54 & 0.91 & 1 & iff0139c1.fits\\
MI04 & 2012-07-17 & 07:21:18 & 0.90 & 1 & iff0140c1.fits\\
MI04 & 2012-07-17 & 07:27:41 & 0.88 & 1 & iff0141c1.fits\\
MI04 & 2012-07-17 & 07:34:04 & 0.88 & 1 & iff0142c1.fits\\
MI04 & 2012-07-17 & 07:40:27 & 0.87 & 1 & iff0143c1.fits\\
MI04 & 2012-07-17 & 07:46:58 & 0.91 & 1 & iff0144c1.fits\\
MI04 & 2012-07-17 & 07:53:24 & 1.11 & 1 & iff0145c1.fits\\
MI04 & 2012-07-17 & 07:59:50 & 1.18 & 1 & iff0146c1.fits finished at airmass ~2.1\\
MI05 & 2012-07-17 & 23:05:14 & 1.26 & 1 & iff0207c1.fits\\
MI05 & 2012-07-17 & 23:11:37 & 1.10 & 1 & iff0208c1.fits\\
MI05 & 2012-07-17 & 23:18:00 & 1.09 & 1 & iff0209c1.fits\\
MI05 & 2012-07-17 & 23:24:23 & 1.04 & 1 & iff0210c1.fits\\
MI05 & 2012-07-17 & 23:30:46 & 1.10 & 1 & iff0211c1.fits\\
MI05 & 2012-07-17 & 23:37:10 & 1.13 & 1 & iff0212c1.fits\\
MI05 & 2012-07-17 & 23:43:34 & 1.06 & 1 & iff0213c1.fits\\
MI05 & 2012-07-17 & 23:49:57 & 0.99 & 1 & iff0214c1.fits\\
MI05 & 2012-07-17 & 23:56:20 & 1.04 & 1 & iff0215c1.fits\\
MI05 & 2012-07-18 & 00:02:43 & 0.92 & 1 & iff0216c1.fits\\
MI05 & 2012-07-18 & 00:09:06 & 0.88 & 1 & iff0217c1.fits\\
MI05 & 2012-07-18 & 00:15:30 & 0.81 & 1 & iff0218c1.fits\\
MI05 & 2012-07-18 & 00:21:53 & 0.99 & 1 & iff0219c1.fits\\
MI05 & 2012-07-18 & 00:28:18 & 0.75 & 1 & iff0220c1.fits\\
MI05 & 2012-07-18 & 00:34:41 & 0.72 & 1 & iff0221c1.fits\\
MI05 & 2012-07-18 & 00:41:04 & 0.78 & 1 & iff0222c1.fits\\
MI05 & 2012-07-18 & 00:47:28 & 0.81 & 1 & iff0223c1.fits\\
MI05 & 2012-07-18 & 00:53:51 & 0.70 & 1 & iff0224c1.fits\\
MI05 & 2012-07-18 & 01:00:14 & 0.62 & 1 & iff0225c1.fits\\
MI05 & 2012-07-18 & 01:06:38 & 0.66 & 1 & iff0226c1.fits\\
MI05 & 2012-07-18 & 01:13:01 & 0.65 & 1 & iff0227c1.fits\\
MI05 & 2012-07-18 & 01:19:24 & 0.74 & 1 & iff0228c1.fits\\
MI05 & 2012-07-18 & 01:25:48 & 0.84 & 1 & iff0229c1.fits\\
MI05 & 2012-07-18 & 01:32:11 & 1.31 & 1 & iff0230c1.fits\\
MI08 & 2012-07-18 & 01:38:37 & 1.33 & 1 & iff0231c1.fits\\
MI08 & 2012-07-18 & 01:45:01 & 1.55 & 1 & iff0232c1.fits\\
MI08 & 2012-07-18 & 01:51:24 & 1.06 & 1 & iff0233c1.fits\\
MI08 & 2012-07-18 & 01:57:47 & 1.09 & 1 & iff0234c1.fits\\
MI08 & 2012-07-18 & 02:04:11 & 1.04 & 1 & iff0235c1.fits\\
MI08 & 2012-07-18 & 02:10:34 & 0.79 & 1 & iff0236c1.fits\\
MI08 & 2012-07-18 & 02:16:57 & 0.84 & 1 & iff0237c1.fits\\
MI08 & 2012-07-18 & 02:23:21 & 0.86 & 1 & iff0238c1.fits\\
MI08 & 2012-07-18 & 02:29:44 & 0.70 & 1 & iff0239c1.fits\\
MI08 & 2012-07-18 & 02:36:08 & 0.60 & 1 & iff0240c1.fits\\
MI08 & 2012-07-18 & 02:42:31 & 0.63 & 1 & iff0241c1.fits\\
MI08 & 2012-07-18 & 02:48:54 & 0.67 & 1 & iff0242c1.fits\\
MI08 & 2012-07-18 & 02:55:18 & 0.71 & 1 & iff0243c1.fits\\
MI08 & 2012-07-18 & 03:01:42 & 0.80 & 1 & iff0244c1.fits\\
MI08 & 2012-07-18 & 03:08:05 & 0.93 & 1 & iff0245c1.fits\\
MI08 & 2012-07-18 & 03:14:28 & 0.77 & 1 & iff0246c1.fits\\
MI08 & 2012-07-18 & 03:20:52 & 0.86 & 1 & iff0247c1.fits\\
MI08 & 2012-07-18 & 03:27:15 & 0.85 & 1 & iff0248c1.fits\\
MI08 & 2012-07-18 & 03:33:38 & 0.97 & 1 & iff0249c1.fits\\
MI08 & 2012-07-18 & 03:40:02 & 0.85 & 1 & iff0250c1.fits\\
MI04 & 2012-07-18 & 03:46:26 & 0.94 & 1 & iff0251c1.fits\\
MI04 & 2012-07-18 & 03:52:50 & 1.00 & 1 & iff0252c1.fits\\
MI04 & 2012-07-18 & 03:59:13 & 1.02 & 1 & iff0253c1.fits\\
MI04 & 2012-07-18 & 04:05:36 & 0.92 & 1 & iff0254c1.fits\\
MI04 & 2012-07-18 & 04:12:00 & 1.03 & 1 & iff0255c1.fits\\
MI04 & 2012-07-18 & 04:18:23 & 1.06 & 1 & iff0256c1.fits\\
MI04 & 2012-07-18 & 04:24:46 & 1.13 & 1 & iff0257c1.fits\\
MI04 & 2012-07-18 & 04:31:10 & 1.13 & 1 & iff0258c1.fits\\
MI04 & 2012-07-18 & 04:37:33 & 1.26 & 1 & iff0259c1.fits\\
MI04 & 2012-07-18 & 04:43:56 & 1.11 & 1 & iff0260c1.fits\\
MI04 & 2012-07-18 & 04:50:19 & 0.98 & 1 & iff0261c1.fits\\
MI04 & 2012-07-18 & 04:56:42 & 1.01 & 1 & iff0262c1.fits\\
MI04 & 2012-07-18 & 05:03:06 & 0.95 & 1 & iff0263c1.fits\\
MI04 & 2012-07-18 & 05:09:29 & 0.99 & 1 & iff0264c1.fits\\
MI04 & 2012-07-18 & 05:15:52 & 0.95 & 1 & iff0265c1.fits\\
MI04 & 2012-07-18 & 05:22:15 & 0.91 & 1 & iff0266c1.fits\\
MI04 & 2012-07-18 & 05:28:38 & 0.93 & 1 & iff0267c1.fits\\
MI04 & 2012-07-18 & 05:35:02 & 0.93 & 1 & iff0268c1.fits\\
MI04 & 2012-07-18 & 05:41:25 & 0.85 & 1 & iff0269c1.fits\\
MI04 & 2012-07-18 & 05:47:48 & 0.77 & 1 & iff0270c1.fits\\
MI03 & 2012-07-18 & 05:54:14 & 0.84 & 1 & iff0271c1.fits\\
MI03 & 2012-07-18 & 06:00:37 & 1.00 & 1 & iff0272c1.fits\\
MI03 & 2012-07-18 & 06:07:00 & 0.98 & 1 & iff0273c1.fits\\
MI03 & 2012-07-18 & 06:13:24 & 1.04 & 1 & iff0274c1.fits\\
MI03 & 2012-07-18 & 06:19:47 & 0.97 & 1 & iff0275c1.fits\\
MI03 & 2012-07-18 & 06:26:10 & 1.10 & 1 & iff0276c1.fits\\
MI03 & 2012-07-18 & 06:32:33 & 1.12 & 1 & iff0277c1.fits\\
MI03 & 2012-07-18 & 06:38:56 & 1.15 & 1 & iff0278c1.fits\\
MI03 & 2012-07-18 & 06:45:19 & 1.25 & 1 & iff0279c1.fits\\
MI03 & 2012-07-18 & 06:51:43 & 1.39 & 1 & iff0280c1.fits\\
MI03 & 2012-07-18 & 06:58:06 & 1.26 & 1 & iff0281c1.fits\\
MI03 & 2012-07-18 & 07:04:30 & 1.32 & 1 & iff0282c1.fits\\
MI03 & 2012-07-18 & 07:10:53 & 1.29 & 1 & iff0283c1.fits\\
MI03 & 2012-07-18 & 07:17:16 & 1.12 & 1 & iff0284c1.fits\\
MI03 & 2012-07-18 & 07:23:39 & 1.07 & 1 & iff0285c1.fits\\
MI03 & 2012-07-18 & 07:30:02 & 1.07 & 1 & iff0286c1.fits\\
MI03 & 2012-07-18 & 07:36:25 & 1.09 & 1 & iff0287c1.fits\\
MI03 & 2012-07-18 & 07:42:49 & 1.17 & 1 & iff0288c1.fits\\
MI03 & 2012-07-18 & 07:49:12 & 1.25 & 1 & iff0289c1.fits\\
MI03 & 2012-07-18 & 07:55:36 & 1.30 & 1 & iff0290c1.fits\\
MI03 & 2012-07-18 & 08:01:59 & 1.43 & 1 & iff0291c1.fits continued to airmass $\sim$2.7\\
MI03 & 2012-07-18 & 08:08:22 & 2.27 & 1 & iff0292c1.fits\\
MI03 & 2012-07-18 & 08:14:46 & 1.82 & 1 & iff0293c1.fits\\
MI03 & 2012-07-18 & 08:21:09 & 1.49 & 1 & iff0294c1.fits\\
MI03 & 2012-07-18 & 08:27:32 & 1.52 & 1 & iff0295c1.fits\\
MI07 & 2012-07-19 & 01:56:12 & 1.88 & 2 & iff0332c1.fits opened after wind went down\\
MI07 & 2012-07-19 & 02:02:36 & 2.13 & 2 & iff0333c1.fits\\
MI07 & 2012-07-19 & 02:08:58 & 2.28 & 2 & iff0334c1.fits\\
MI07 & 2012-07-19 & 02:15:22 & 1.95 & 2 & iff0335c1.fits\\
MI07 & 2012-07-19 & 02:21:45 & 2.03 & 2 & iff0336c1.fits\\
MI07 & 2012-07-19 & 02:28:09 & 2.32 & 2 & iff0337c1.fits\\
MI07 & 2012-07-19 & 02:34:32 & 2.34 & 2 & iff0338c1.fits\\
MI07 & 2012-07-19 & 02:40:55 & 1.79 & 2 & iff0339c1.fits\\
MI07 & 2012-07-19 & 02:47:19 & 1.81 & 2 & iff0340c1.fits\\
MI07 & 2012-07-19 & 02:53:42 & 1.48 & 2 & iff0341c1.fits\\
MI07 & 2012-07-19 & 03:00:05 & 1.18 & 2 & iff0342c1.fits\\
MI07 & 2012-07-19 & 03:06:28 & 1.49 & 2 & iff0343c1.fits\\
MI07 & 2012-07-19 & 03:12:51 & 1.55 & 2 & iff0344c1.fits\\
MI07 & 2012-07-19 & 03:19:14 & 1.62 & 2 & iff0345c1.fits\\
MI07 & 2012-07-19 & 03:25:37 & 1.62 & 2 & iff0346c1.fits\\
MI07 & 2012-07-19 & 03:32:00 & 2.31 & 2 & iff0347c1.fits\\
MI07 & 2012-07-19 & 03:38:24 & 2.09 & 2 & iff0348c1.fits\\
MI07 & 2012-07-19 & 03:44:47 & 1.65 & 2 & iff0349c1.fits\\
MI07 & 2012-07-19 & 03:51:10 & 2.10 & 2 & iff0350c1.fits\\
MI07 & 2012-07-19 & 03:57:34 & 2.75 & 2 & iff0351c1.fits\\
MI07 & 2012-07-19 & 04:03:57 & 2.37 & 2 & iff0352c1.fits\\
MI07 & 2012-07-19 & 04:10:20 & 1.76 & 2 & iff0353c1.fits\\
MI07 & 2012-07-19 & 04:16:43 & 1.35 & 2 & iff0354c1.fits\\
MI07 & 2012-07-19 & 04:23:06 & 1.29 & 2 & iff0355c1.fits\\
MI07 & 2012-07-19 & 04:29:29 & 1.63 & 2 & iff0356c1.fits\\
MI07 & 2012-07-19 & 04:35:53 & 1.68 & 2 & iff0357c1.fits\\
MI07 & 2012-07-19 & 04:42:16 & 1.44 & 2 & iff0358c1.fits\\
MI07 & 2012-07-19 & 04:48:39 & 1.39 & 2 & iff0359c1.fits\\
MI07 & 2012-07-19 & 04:55:02 & 1.16 & 2 & iff0360c1.fits\\
MI07 & 2012-07-19 & 05:01:25 & 1.59 & 2 & iff0361c1.fits\\
MI07 & 2012-07-19 & 05:07:52 & 1.26 & 2 & iff0362c1.fits\\
MI07 & 2012-07-19 & 05:14:16 & 1.12 & 2 & iff0363c1.fits seeing extremely variable whole night.\\
MI07 & 2012-07-20 & 00:34:05 & 0.65 & 1 & iff0364c1.fits\\
MI07 & 2012-07-20 & 00:40:28 & 0.69 & 1 & iff0365c1.fits\\
MI07 & 2012-07-20 & 00:46:51 & 0.64 & 1 & iff0366c1.fits\\
MI07 & 2012-07-20 & 00:53:14 & 0.76 & 1 & iff0367c1.fits\\
MI07 & 2012-07-20 & 00:59:38 & 0.86 & 1 & iff0368c1.fits\\
MI07 & 2012-07-20 & 01:06:02 & 0.72 & 1 & iff0369c1.fits\\
MI07 & 2012-07-20 & 01:12:25 & 0.80 & 1 & iff0370c1.fits\\
MI07 & 2012-07-20 & 01:18:48 & 0.82 & 1 & iff0371c1.fits\\
MI07 & 2012-07-20 & 01:25:12 & 0.99 & 1 & iff0372c1.fits\\
MI07 & 2012-07-20 & 01:31:35 & 1.06 & 1 & iff0373c1.fits\\
MI07 & 2012-07-20 & 01:37:58 & 0.95 & 1 & iff0374c1.fits\\
MI07 & 2012-07-20 & 01:44:22 & 1.02 & 1 & iff0375c1.fits\\
MI07 & 2012-07-20 & 01:50:45 & 1.02 & 1 & iff0376c1.fits\\
MI07 & 2012-07-20 & 01:57:08 & 0.82 & 1 & iff0377c1.fits\\
MI07 & 2012-07-20 & 02:03:31 & 0.85 & 1 & iff0378c1.fits\\
MI07 & 2012-07-20 & 02:09:55 & 0.89 & 1 & iff0379c1.fits\\
MI07 & 2012-07-20 & 02:16:18 & 0.97 & 1 & iff0380c1.fits\\
MI07 & 2012-07-20 & 02:22:41 & 0.97 & 1 & iff0381c1.fits\\
MI07 & 2012-07-20 & 02:29:04 & 1.04 & 1 & iff0382c1.fits\\
MI07 & 2012-07-20 & 02:35:27 & 0.99 & 1 & iff0383c1.fits\\
MI08 & 2012-07-20 & 02:42:46 & 0.90 & 1 & iff0384c1.fits\\
MI08 & 2012-07-20 & 02:49:09 & 0.58 & 1 & iff0385c1.fits\\
MI08 & 2012-07-20 & 02:55:33 & 0.62 & 1 & iff0386c1.fits\\
MI08 & 2012-07-20 & 03:01:56 & 0.81 & 1 & iff0387c1.fits\\
MI08 & 2012-07-20 & 03:08:19 & 0.75 & 1 & iff0388c1.fits\\
MI08 & 2012-07-20 & 03:14:42 & 0.73 & 1 & iff0389c1.fits\\
MI08 & 2012-07-20 & 03:21:06 & 0.61 & 1 & iff0390c1.fits\\
MI08 & 2012-07-20 & 03:27:29 & 0.66 & 1 & iff0391c1.fits\\
MI08 & 2012-07-20 & 03:33:52 & 0.77 & 1 & iff0392c1.fits\\
MI08 & 2012-07-20 & 03:40:16 & 0.68 & 1 & iff0393c1.fits\\
MI08 & 2012-07-20 & 03:46:39 & 0.70 & 1 & iff0394c1.fits\\
MI08 & 2012-07-20 & 03:53:02 & 0.94 & 1 & iff0395c1.fits\\
MI08 & 2012-07-20 & 03:59:26 & 1.00 & 1 & iff0396c1.fits\\
MI08 & 2012-07-20 & 04:05:49 & 0.85 & 1 & iff0397c1.fits\\
MI08 & 2012-07-20 & 04:12:12 & 0.84 & 1 & iff0398c1.fits\\
MI08 & 2012-07-20 & 04:18:36 & 0.83 & 1 & iff0399c1.fits\\
MI08 & 2012-07-20 & 04:24:59 & 0.86 & 1 & iff0400c1.fits\\
MI08 & 2012-07-20 & 04:31:22 & 0.94 & 1 & iff0401c1.fits\\
MI08 & 2012-07-20 & 04:37:46 & 0.87 & 1 & iff0402c1.fits\\
MI08 & 2012-07-20 & 04:44:10 & 0.85 & 1 & iff0403c1.fits\\
MI01 & 2012-07-20 & 04:50:42 & 0.85 & 1 & iff0404c1.fits\\
MI01 & 2012-07-20 & 04:57:06 & 0.77 & 1 & iff0405c1.fits\\
MI01 & 2012-07-20 & 05:03:29 & 0.86 & 1 & iff0406c1.fits\\
MI01 & 2012-07-20 & 05:09:52 & 0.73 & 1 & iff0407c1.fits\\
MI01 & 2012-07-20 & 05:16:16 & 0.71 & 1 & iff0408c1.fits\\
MI01 & 2012-07-20 & 05:22:39 & 0.63 & 1 & iff0409c1.fits\\
MI01 & 2012-07-20 & 05:29:02 & 0.70 & 1 & iff0410c1.fits\\
MI01 & 2012-07-20 & 05:35:25 & 0.69 & 1 & iff0411c1.fits\\
MI01 & 2012-07-20 & 05:41:48 & 0.73 & 1 & iff0412c1.fits\\
MI01 & 2012-07-20 & 05:48:11 & 0.73 & 1 & iff0413c1.fits\\
MI01 & 2012-07-20 & 05:54:35 & 0.83 & 1 & iff0414c1.fits\\
MI01 & 2012-07-20 & 06:00:58 & 0.78 & 1 & iff0415c1.fits\\
MI04 & 2012-07-21 & 00:32:55 & 1.17 & 1 & iff0459c2.fits\\
MI04 & 2012-07-21 & 00:39:18 & 1.23 & 1 & iff0460c2.fits\\
MI04 & 2012-07-21 & 00:45:42 & 1.05 & 1 & iff0461c2.fits\\
MI04 & 2012-07-21 & 00:52:05 & 0.99 & 1 & iff0462c2.fits\\
MI04 & 2012-07-21 & 00:58:29 & 1.06 & 1 & iff0463c2.fits\\
MI04 & 2012-07-21 & 01:04:52 & 0.99 & 1 & iff0464c2.fits\\
MI04 & 2012-07-21 & 01:11:16 & 1.19 & 1 & iff0465c2.fits\\
MI04 & 2012-07-21 & 01:17:39 & 0.98 & 1 & iff0466c2.fits\\
MI04 & 2012-07-21 & 01:24:43 & 1.03 & 1 & iff0467c2.fits\\
MI04 & 2012-07-21 & 01:33:24 & 1.15 & 1 & iff0468c2.fits\\
MI04 & 2012-07-21 & 01:37:02 & 1.24 & 1 & iff0469c2.fits\\
MI04 & 2012-07-21 & 01:43:30 & 1.07 & 1 & iff0470c2.fits\\
MI04 & 2012-07-21 & 02:18:10 & 0.77 & 1 & iff0471c2.fits\\
MI04 & 2012-07-21 & 02:24:33 & 0.97 & 1 & iff0472c2.fits\\
MI04 & 2012-07-21 & 02:30:57 & 0.69 & 1 & iff0473c2.fits\\
MI04 & 2012-07-21 & 02:37:20 & 0.83 & 1 & iff0474c2.fits\\
MI04 & 2012-07-21 & 02:43:44 & 0.75 & 1 & iff0475c2.fits\\
MI04 & 2012-07-21 & 02:50:07 & 0.89 & 1 & iff0476c2.fits\\
MI04 & 2012-07-21 & 02:56:30 & 0.77 & 1 & iff0477c2.fits\\
MI04 & 2012-07-21 & 03:02:53 & 0.72 & 1 & iff0478c2.fits\\
MI04 & 2012-07-21 & 03:09:16 & 0.75 & 1 & iff0479c2.fits\\
MI03 & 2012-07-21 & 03:17:43 & 0.76 & 1 & iff0480c2.fits\\
MI03 & 2012-07-21 & 03:24:06 & 0.69 & 1 & iff0481c2.fits\\
MI03 & 2012-07-21 & 03:30:29 & 0.75 & 1 & iff0482c2.fits\\
MI03 & 2012-07-21 & 03:36:53 & 0.76 & 1 & iff0483c2.fits\\
MI03 & 2012-07-21 & 03:43:16 & 0.81 & 1 & iff0484c2.fits\\
MI03 & 2012-07-21 & 03:49:39 & 1.06 & 1 & iff0485c2.fits\\
MI03 & 2012-07-21 & 03:56:03 & 0.83 & 1 & iff0486c2.fits\\
MI03 & 2012-07-21 & 04:02:26 & 0.88 & 1 & iff0487c2.fits\\
MI03 & 2012-07-21 & 04:08:49 & 0.87 & 1 & iff0488c2.fits\\
MI03 & 2012-07-21 & 04:15:12 & 1.02 & 1 & iff0489c2.fits\\
MI03 & 2012-07-21 & 04:21:35 & 0.97 & 1 & iff0490c2.fits\\
MI03 & 2012-07-21 & 04:27:59 & 0.88 & 1 & iff0491c2.fits\\
MI03 & 2012-07-21 & 04:34:22 & 0.92 & 1 & iff0492c2.fits\\
MI03 & 2012-07-21 & 04:40:46 & 1.16 & 1 & iff0493c2.fits\\
MI03 & 2012-07-21 & 04:47:09 & 1.07 & 1 & iff0494c2.fits\\
MI03 & 2012-07-21 & 04:53:32 & 1.07 & 1 & iff0495c2.fits\\
MI03 & 2012-07-21 & 04:59:55 & 1.07 & 1 & iff0496c2.fits\\
MI03 & 2012-07-21 & 05:06:19 & 1.07 & 1 & iff0497c2.fits\\
MI03 & 2012-07-21 & 05:12:42 & 0.91 & 1 & iff0498c2.fits\\
MI03 & 2012-07-21 & 05:19:04 & 0.91 & 1 & iff0499c2.fits\\
MI03 & 2012-07-21 & 05:25:28 & 0.85 & 1 & iff0500c2.fits\\
MI03 & 2012-07-21 & 05:31:51 & 0.84 & 1 & iff0501c2.fits\\
MI03 & 2012-07-21 & 05:38:15 & 0.89 & 1 & iff0502c2.fits\\
MI03 & 2012-07-21 & 05:44:38 & 0.86 & 1 & iff0503c2.fits\\
MI04 & 2012-07-21 & 05:51:15 & 0.78 & 1 & iff0504c2.fits\\
MI04 & 2012-07-21 & 05:57:38 & 0.78 & 1 & iff0505c2.fits\\
MI04 & 2012-07-21 & 06:04:02 & 0.77 & 1 & iff0506c2.fits\\
MI04 & 2012-07-21 & 06:10:33 & 0.85 & 1 & iff0507c2.fits\\
MI05 & 2012-07-21 & 23:00:35 & 1.61 & 2 & iff0509c2.fits clouds\\
MI05 & 2012-07-21 & 23:07:05 & 1.37 & 2 & iff0510c2.fits\\
MI05 & 2012-07-21 & 23:13:28 & 1.23 & 2 & iff0511c2.fits\\
MI05 & 2012-07-21 & 23:19:52 & 1.22 & 2 & iff0512c2.fits\\
MI05 & 2012-07-21 & 23:26:15 & 1.45 & 2 & iff0513c2.fits\\
MI05 & 2012-07-21 & 23:32:38 & 1.20 & 2 & iff0514c2.fits\\
MI05 & 2012-07-21 & 23:39:02 & 0.84 & 2 & iff0515c2.fits\\
MI05 & 2012-07-21 & 23:45:25 & 1.08 & 2 & iff0516c2.fits\\
MI05 & 2012-07-21 & 23:51:48 & 1.05 & 2 & iff0517c2.fits\\
MI05 & 2012-07-21 & 23:58:11 & 1.29 & 2 & iff0518c2.fits\\
MI05 & 2012-07-22 & 00:04:34 & 1.13 & 2 & iff0519c2.fits\\
MI05 & 2012-07-22 & 00:10:58 & 1.08 & 2 & iff0520c2.fits\\
MI05 & 2012-07-22 & 00:17:22 & 1.02 & 2 & iff0521c2.fits\\
MI05 & 2012-07-22 & 00:23:45 & 1.12 & 2 & iff0522c2.fits\\
MI05 & 2012-07-22 & 00:30:09 & 1.02 & 2 & iff0523c2.fits\\
MI05 & 2012-07-22 & 00:36:33 & 0.96 & 2 & iff0524c2.fits\\
MI05 & 2012-07-22 & 00:42:56 & 1.32 & 2 & iff0525c2.fits\\
MI05 & 2012-07-22 & 00:49:20 & 1.17 & 2 & iff0526c2.fits\\
MI05 & 2012-07-22 & 00:55:43 & 1.36 & 2 & iff0527c2.fits\\
MI05 & 2012-07-22 & 01:02:06 & 1.03 & 2 & iff0528c2.fits\\
MI05 & 2012-07-22 & 01:09:00 & 0.84 & 2 & iff0529c2.fits\\
MI05 & 2012-07-22 & 01:15:24 & 0.86 & 2 & iff0530c2.fits\\
MI05 & 2012-07-22 & 01:21:48 & 1.00 & 2 & iff0531c2.fits\\
MI05 & 2012-07-22 & 01:28:11 & 0.87 & 2 & iff0532c2.fits\\
MI05 & 2012-07-22 & 01:34:34 & 1.15 & 2 & iff0533c2.fits\\
MI05 & 2012-07-22 & 01:40:58 & 1.03 & 2 & iff0534c2.fits\\
MI05 & 2012-07-22 & 01:47:21 & 1.03 & 2 & iff0535c2.fits\\
MI05 & 2012-07-22 & 01:53:44 & 1.21 & 2 & iff0536c2.fits\\
MI05 & 2012-07-22 & 02:00:07 & 1.12 & 2 & iff0537c2.fits\\
MI05 & 2012-07-22 & 02:06:31 & 1.16 & 2 & iff0538c2.fits clouds not a problem\\
MI06 & 2012-07-22 & 02:12:54 & 0.80 & 1 & iff0539c2.fits\\
MI06 & 2012-07-22 & 02:19:17 & 0.88 & 1 & iff0540c2.fits\\
MI06 & 2012-07-22 & 02:25:40 & 0.88 & 1 & iff0541c2.fits\\
MI06 & 2012-07-22 & 02:32:04 & 1.04 & 1 & iff0542c2.fits\\
MI06 & 2012-07-22 & 02:38:27 & 1.05 & 1 & iff0543c2.fits\\
MI06 & 2012-07-22 & 02:44:50 & 0.94 & 1 & iff0544c2.fits\\
MI06 & 2012-07-22 & 02:51:14 & 0.92 & 1 & iff0545c2.fits\\
MI06 & 2012-07-22 & 02:57:38 & 0.82 & 1 & iff0546c2.fits\\
MI06 & 2012-07-22 & 03:04:01 & 0.93 & 1 & iff0547c2.fits\\
MI06 & 2012-07-22 & 03:10:25 & 0.93 & 1 & iff0548c2.fits\\
MI06 & 2012-07-22 & 03:16:48 & 0.82 & 1 & iff0549c2.fits\\
MI06 & 2012-07-22 & 03:23:11 & 1.06 & 1 & iff0550c2.fits\\
MI06 & 2012-07-22 & 03:29:35 & 1.03 & 1 & iff0551c2.fits\\
MI06 & 2012-07-22 & 03:35:58 & 1.11 & 1 & iff0552c2.fits\\
MI06 & 2012-07-22 & 03:42:21 & 0.83 & 1 & iff0553c2.fits\\
MI06 & 2012-07-22 & 03:48:45 & 0.77 & 1 & iff0554c2.fits\\
MI06 & 2012-07-22 & 03:55:08 & 0.85 & 1 & iff0555c2.fits\\
MI07 & 2012-07-22 & 04:01:37 & 1.18 & 1 & iff0556c2.fits\\
MI07 & 2012-07-22 & 04:08:00 & 1.66 & 1 & iff0557c2.fits\\
MI07 & 2012-07-22 & 04:14:24 & 1.82 & 1 & iff0558c2.fits\\
MI07 & 2012-07-22 & 04:20:47 & 1.68 & 1 & iff0559c2.fits\\
MI07 & 2012-07-22 & 04:27:10 & 1.69 & 1 & iff0560c2.fits\\
MI07 & 2012-07-22 & 04:33:34 & 1.51 & 1 & iff0561c2.fits\\
MI07 & 2012-07-22 & 04:39:57 & 1.27 & 1 & iff0562c2.fits\\
MI07 & 2012-07-22 & 04:46:20 & 1.09 & 1 & iff0563c2.fits\\
MI07 & 2012-07-22 & 04:52:43 & 1.28 & 1 & iff0564c2.fits\\
MI07 & 2012-07-22 & 04:59:07 & 1.13 & 1 & iff0565c2.fits\\
MI07 & 2012-07-22 & 05:05:31 & 1.10 & 1 & iff0566c2.fits\\
MI07 & 2012-07-22 & 05:11:54 & 1.18 & 1 & iff0567c2.fits\\
MI07 & 2012-07-22 & 05:18:18 & 1.14 & 1 & iff0568c2.fits\\
MI07 & 2012-07-22 & 05:24:41 & 1.21 & 1 & iff0569c2.fits\\
MI07 & 2012-07-22 & 05:31:04 & 1.14 & 1 & iff0570c2.fits\\
MI07 & 2012-07-22 & 05:37:28 & 1.20 & 1 & iff0571c2.fits\\
MI07 & 2012-07-22 & 05:43:51 & 1.18 & 1 & iff0572c2.fits\\
MI07 & 2012-07-22 & 05:50:15 & 1.30 & 1 & iff0573c2.fits\\
MI07 & 2012-07-22 & 05:56:38 & 1.16 & 1 & iff0574c2.fits\\
MI07 & 2012-07-22 & 06:03:02 & 1.20 & 1 & iff0575c2.fits\\
MI07 & 2012-07-23 & 00:28:24 & 0.92 & 1 & iff0576c2.fits\\
MI07 & 2012-07-23 & 00:34:54 & 0.77 & 1 & iff0577c2.fits\\
MI07 & 2012-07-23 & 00:41:17 & 0.82 & 1 & iff0578c2.fits\\
MI07 & 2012-07-23 & 00:47:41 & 0.71 & 1 & iff0579c2.fits\\
MI07 & 2012-07-23 & 00:54:04 & 0.74 & 1 & iff0580c2.fits\\
MI07 & 2012-07-23 & 01:00:27 & 0.82 & 1 & iff0581c2.fits\\
MI07 & 2012-07-23 & 01:06:51 & 0.79 & 1 & iff0582c2.fits\\
MI07 & 2012-07-23 & 01:13:15 & 0.81 & 1 & iff0583c2.fits\\
MI07 & 2012-07-23 & 01:19:38 & 0.85 & 1 & iff0584c2.fits\\
MI07 & 2012-07-23 & 01:26:01 & 0.82 & 1 & iff0585c2.fits\\
MI07 & 2012-07-23 & 01:32:24 & 0.80 & 1 & iff0586c2.fits\\
MI07 & 2012-07-23 & 01:38:48 & 0.70 & 1 & iff0587c2.fits\\
MI07 & 2012-07-23 & 01:45:11 & 0.59 & 1 & iff0588c2.fits\\
MI07 & 2012-07-23 & 01:51:34 & 0.65 & 1 & iff0589c2.fits\\
MI07 & 2012-07-23 & 01:57:58 & 0.69 & 1 & iff0590c2.fits\\
MI07 & 2012-07-23 & 02:04:21 & 0.64 & 1 & iff0591c2.fits\\
MI07 & 2012-07-23 & 02:10:44 & 0.57 & 1 & iff0592c2.fits\\
MI07 & 2012-07-23 & 02:17:08 & 0.60 & 1 & iff0593c2.fits\\
MI07 & 2012-07-23 & 02:23:31 & 0.61 & 1 & iff0594c2.fits\\
MI07 & 2012-07-23 & 02:29:54 & 0.62 & 1 & iff0595c2.fits\\
MI05 & 2012-07-23 & 02:36:32 & 0.74 & 1 & iff0596c2.fits\\
MI05 & 2012-07-23 & 02:45:01 & 0.74 & 1 & iff0597c2.fits\\
MI05 & 2012-07-23 & 02:51:24 & 0.69 & 1 & iff0598c2.fits\\
MI05 & 2012-07-23 & 02:57:47 & 0.59 & 1 & iff0599c2.fits\\
MI05 & 2012-07-23 & 03:04:10 & 0.64 & 1 & iff0600c2.fits\\
MI05 & 2012-07-23 & 03:10:34 & 0.66 & 1 & iff0601c2.fits\\
MI05 & 2012-07-23 & 03:16:57 & 0.72 & 1 & iff0602c2.fits\\
MI05 & 2012-07-23 & 03:23:21 & 0.77 & 1 & iff0603c2.fits\\
MI05 & 2012-07-23 & 03:29:45 & 0.76 & 1 & iff0604c2.fits\\
MI05 & 2012-07-23 & 03:36:08 & 0.76 & 1 & iff0605c2.fits\\
MI05 & 2012-07-23 & 03:42:32 & 0.81 & 1 & iff0606c2.fits\\
MI05 & 2012-07-23 & 03:48:55 & 0.86 & 1 & iff0607c2.fits\\
MI05 & 2012-07-23 & 03:55:18 & 0.85 & 1 & iff0608c2.fits\\
MI05 & 2012-07-23 & 04:01:42 & 0.80 & 1 & iff0609c2.fits\\
MI05 & 2012-07-23 & 04:08:05 & 0.75 & 1 & iff0610c2.fits\\
MI05 & 2012-07-23 & 04:14:29 & 0.82 & 1 & iff0611c2.fits\\
MI05 & 2012-07-23 & 04:20:52 & 0.71 & 1 & iff0612c2.fits\\
MI05 & 2012-07-23 & 04:27:15 & 0.75 & 1 & iff0613c2.fits\\
SJ02&2012-08-13&05:52&0.9&1&\\
SJ03&2012-08-13&07:45&0.8&1&\\
SJ02&2012-08-13&08:42&1.2&1&\\
SJ03&2012-08-13&09:38&1.6&1&\\
SJ02&2012-08-14&06:00&2.1&1&\\
SJ03&2012-08-14&07:04&1.9&1&\\
SJ02&2012-08-14&08:05&2.5&1&\\
SJ03&2012-08-14&09:06&3.0&1&\\
SJ02&2012-08-14&10:07&3.4&1&\\
SJ03&2012-08-15&07:03&2.9&1&\\
SJ02&2012-08-15&08:08&3.4&1&\\
SJ03&2012-08-15&09:04&3.9&1&\\
SJ02&2012-08-16&06:06&1.7&1& visit truncated by instrument problem\\
SJ03&2012-08-16&07:15&1.5&1& shortened visit\\
SJ02&2012-08-16&08:06&1.6&1&\\
SJ03&2012-08-16&09:04&1.8&1&\\
SJ02&2012-08-16&10:03&1.9&1&\\
ML01&130603&04:36&0.52&1& 0.5-0.55${^\prime^\prime}$   Engineering time\\
ML01&130603&04:53&0.52&1& 0.5-0.55${^\prime^\prime}$\\
ML01&130603&05:10&0.52&1& 0.5-0.55${^\prime^\prime}$\\
ML01&130603&05:27&0.52&1& 0.5-0.55${^\prime^\prime}$\\
ML02&130603&05:56&0.57&1& 0.55-0.6${^\prime^\prime}$ at least good for template creation\\
ML02&130603&06:09&0.57&1& 0.55-0.6${^\prime^\prime}$ \\
ML01&130603&06:24&0.55&1& 0.5-0.6${^\prime^\prime}$ \\
ML01&130603&06:39&0.55&1& 0.5-0.6${^\prime^\prime}$ \\
ML01&130604&04:39&.50&1&\\
ML01&130604&04:58&.47&1& .45-.50 \\
ML01&130604&05:09&.47&1& .45-.50  seeing getting slightly better.\\
ML01&130604&05:22&.47&1& .45-.50\\
ML02&130604&05:36&.45&1& change fields and re-do wavefront\\
ML02&130604&05:51&.45&1& \\
ML02&130604&06:06&.45&1& steady conditions \\
ML01&130604&06:32&.45&1& change fields and re-do wavefront\\
ML01&130604&06:47&.45&1&\\
ML01&130604&07:03&.47&1& .45-.50\\
ML02&130604&07:30&.47&1& change fields and re-do wavefront  .45-.50\\
ML02&130604&07:43&.50&1& detector hung, restart guiding. few seconds lost\\
ML02&130604&07:59&.55&1& seeing slowly getting worse \\
ML01&130604&08:21&.50&1& change fields and re-do wavefront\\
ML01&130604&08:36&.55&1& \\
ML01&130604&08:48&.55&1& moon rising, bkg level rising slightly \\
ML02&130604&09:14&.60&1& change fields and re-do wavefront\\
ML02&130604&09:27&.65&1& possible differential refraction  \\
ML02&130604&09:43&.75&1& \\
ML02&130604&10:02&.65&1& single frame in R to look at differential refraction\\
ML02&130605&04:57&0.75&1&  \\
ML02&130605&05:04&0.7&1&  \\
ML02&130605&05:16&0.65&1&  seeing getting better\\
ML03&130605&05:41&0.55&1&  change field and re-do wavefront\\
ML03&130605&05:56&0.55&1& \\
ML03&130605&06:08&0.55&1& \\
ML02&130605&06:26&0.5&1&  change field and re-do wavefront\\
ML02&130605&06:39&0.6&1& \\
ML02&130605&06:52&0.65&1&  server crashed at 07:02 lost several minutes\\
ML03&130605&07:10&0.7&1& change field and re-do wavefront, change to 15 exp.\\
ML03&130605&07:36&0.65&1& \\
ML03&130605&07:39&0.65&1& \\
ML02&130605&07:53&0.8&1&  change field and re-do wavefront. thin clouds, seeing deteriorating\\
ML02&130605&08:09&0.85&1&  error during readout of 5151, exp. lost\\
ML03&130605&08:33&0.7&1& change field and re-do wavefront \\
ML03&130605&08:45&0.8&1& \\
ML03&130605&09:00&0.85&1&  \\
ML02&130605&09:20&0.85&1&  change field, re-do wavefront; change filter to r \\
ML02&130605&09:33&0.9&1&  moon rising\\
ML02&130605&09:16&1.0&1&  seeing deteriorating, and variable\\
ML02&130605&10:11&1.4&2&  redo wave front. stopped taking data, seeing  too bad\\
ML02&130606&04:44&.75&1& redo wavefront calibrations, exp. 5337 lost\\
ML02&130606&05:00&.7&1&\\
ML02&130606&05:12&.7&1& made up extra frame here\\
ML03&130606&05:32&.65&1&\\
ML03&130606&05:47&.7&1& seeing variable\\
ML03&130606&05:59&.75&1&\\
ML02&130606&06:15&.6&1&\\
ML02&130606&06:31&.55&1&\\
ML02&130606&06:42&.75&1& seeing highly variable\\
ML03&130606&06:57&.65&1&\\
ML03&130606&07:07&.7&1& seeing still varible\\
ML03&130606&07:20&.75&1&\\
ML02&130606&07:39&.7&1&\\
ML02&130606&07:52&.7&1&\\
ML02&130606&08:02&.8&1&\\
ML03&130606&08:23&.7&1&\\
ML03&130606&08:36&.7&1&\\
ML03&130606&08:48&.9&1& seeing is deteriorating, extra frames\\
ML03&130606&09:01&.8&1&\\
ML02&130606&09:18&1.0&1& changed to r filter, thin clouds moving in.\\
ML02&130606&09:40&1.0&1& recalibrate wave front\\
ML02&130606&09:53&1.2&1&\\
ML02&130607&03:32&.55&1& psf slightly off - atmospheric refraction, better as field rises  \\
ML02&130607&03:47&.5&1&  \\
ML02&130607&04:02&.5&1&  \\
ML02&130607&04:15&.5&1& redo wavefront calibrations. exp. 5554 lost \\
ML00&130607&04:27&.5&1&  \\
ML02&130607&04:42&.45&1&  \\
ML02&130607&04:57&.5&1&  \\
ML02&130607&05:10&.5&1&  \\
ML00&130607&05:22&.45&1&  \\
ML02&130607&05:37&.45&1&  \\
ML02&130607&05:52&.4&1& Amazing seeing! several frames $<$ .4${^\prime^\prime}$ \\
ML02&130607&06:10&.4&1&\\
ML01&130608&03:42&.75&1&  \\
ML01&130608&03:57&.7&1& redo wavefront exp. 5702 lost \\
ML01&130608&04:14&.65&1& conditions improving and becoming somewhat stable \\
ML01&130608&04:29&.65&1& \\
ML01&130608&04:44&.65&1& \\
ML01&130608&04:59&.75&1& redo wave front \\
ML01&130608&05:05&.8&1& seeing getting worse \\
ML01&130608&05:23&.85&1&  \\
ML01&130608&05:38&.7&1& highly variable seeing. redo wave front \\
ML01&130608&06:01&.75&1& \\
ML01&130608&06:17&.85&1& redo wave front exp. 5754 lost \\
ML01&130608&06:34&.75&1& very high winds\\
ML03&130609&03:38&.65&1& seeing getting worse\\
ML03&130609&03:53&.65&1& \\
ML03&130609&04:05&.65&1& \\
ML03&130609&04:21&.6&1& redo wavefront\\
ML03&130609&04:32&.7&1& bad clouds on 5892\\
ML03&130609&04:48&.6&1& seeing becoming varaible, clouds moving in at end\\
ML03&130609&04:59&1.2&2& bad clouds starting on 5901. no guiding. unuseable\\
ML03&130609&05:14&1.0&2& bad clouds. no guiding. likely unuseable. redo wavefront. exp. 5913 lost\\
ML03&130609&05:48&.7-1.2&2& highly variable conditions. some may be useable\\
ML03&130609&06:01&.6&1& clouds cleared\\
ML03&130609&06:20&.55&1& redo wavefront\\
ML03&130609&06:45&.6&1& clouds coming back, slightly variable conditions\\
ML03&130609&07:00&.6&1& clouds gone\\
ML03&130609&07:15&.6&1& \\
ML03&130609&07:28&.6&1& redo wavefront\\
ML03&130609&07:40&.65&1& \\
ML03&130609&07:56&.7&1& \\
ML03&130609&08:08&.8&1& \\
ML03&130609&08:21&.65&1&\\
ML01&130610&05:10&.55&2& only 20\% flux due to clouds, may be useable\\
ML01&130610&05:25&.55&2& \\
ML01&130610&05:37&.55&2& slightly better fluxes in 6091 & 6092, still 1 mag off\\
ML01&130610&05:50&.55&2& stay on this field until fluxes improve\\
ML01&130610&06:03&.5&2& clouds still taking flux\\
ML01&130610&06:18&.5&2& \\
ML01&130610&06:31&.55&2& \\
ML01&130610&06:43&.5&3& very low fluxes\\
ML01&130610&06:56&.5&3& about 4 mag extinction\\
ML01&130610&07:08&.5&2& \\
ML01&130610&07:21&.5&2& \\
ML01&130610&07:34&.5&2& \\
ML04&130610&07:48&.6&2& change fields. still bad clouds\\
ML04&130610&08:03&.6&2& \\
ML04&130610&08:18&.6&2& clouds still bad. redo wavefront, no help.\\
ML01&130611&04:51&.85&1& good fluxes, marginal seeing\\
ML01&130611&05:09&.85&1& \\
ML01&130611&05:19&.8&1& \\
ML03&130611&05:36&.8&1& redo wavefront\\
ML03&130611&05:43&.7&1& \\
ML03&130611&06:01&.7&1& \\
ML01&130611&06:22&.65&1& redo wavefront\\
ML01&130611&06:37&.65&1& \\
ML01&130611&06:55&.8&1& \\
ML03&130611&07:09&.9&1& redo wavefront\\
ML03&130611&07:24&.8&1& \\
ML03&130611&07:37&.8&1& \\
ML01&130611&07:56&.8&1& redo wavefront \\
ML01&130611&08:11&.9&1& redo wavefront\\
ML01&130611&08:29&.75&1& some elongation on end frame\\
ML03&130611&08:47&.7&1& some elongation\\
ML03&130611&09:02&.7&1& atomsphereic refraction getting worse\\
ML03&130611&09:15&.8&1& \\
ML02&130611&09:35&.9&1& R filter. redo wavefront. high airmass. 6382 lost, 6383 focus issue\\
ML02&130611&09:52&.8&1& \\
ML02&130611&10:05&.8&1&\\
ML01&130612&04:43&.85&2& not photometric, variable seeing\\
ML01&130612&04:55&.9&2& \\
ML01&130612&05:03&.85&2& losing $\sim$20\% of flux \\
ML01&130612&05:21&.95&2& up to 30\% flux loss in some frames\\
ML03&130612&05:38&.95&2& redo wavefront, up to 50\% flux loss\\
ML03&130612&05:50&1.0&2& \\
ML03&130612&06:00&1.3&2& very high flux loss. likely unusable\\
ML03&130612&06:15&.9&2& \\
ML01&130612&06:32&.85&2& redo wavefront. somewhat better fluxes\\
ML01&130612&06:45&.85&2& \\
ML01&130612&06:55&.8&2& fluxes getting better at 3541 but still a big loss\\
ML01&130612&07:10&.95&2& \\
ML03&130612&07:27&1.1&2& redo wavefront. fluxes back down \\
ML03&130612&07:40&1.0&2& \\
ML03&130612&07:50&1.0&2& \\
ML03&130612&08:05&1.0&2& \\
ML01&130612&08:21&1.2&2& redo wavefront\\
ML01&130612&08:34&1.3&2& \\
ML01&130612&08:44&1.4&2& stopped taking data early. likely useless.\\
ML01&130613&04:49&.65&1& some high clouds, but flux is okay\\
ML01&130613&05:03&.75&1& redo waverfront, minor astigmatism\\
ML01&130613&05:18&.7&1& \\
ML03&130613&05:33&.55&1& \\
ML03&130613&05:47&.55&1& \\
ML03&130613&05:59&.7&1& \\
ML01&130613&06:19&.65&1& redo wavefront\\
ML01&130613&06:32&.65&1& \\
ML01&130613&06:45&.75&1& \\
ML03&130613&07:04&.6&1& redo wavefront\\
ML03&130613&07:16&.7&1& up to 30\% variation/high clouds, total flux not majorly impacted\\
ML03&130613&07:29&.75&1& \\
ML01&130613&07:49&.7&1& redo wavefront\\
ML01&130613&08:02&.8&1& pause for clouds. 6771 like unuseable due to clouds\\
ML01&130613&08:47&.75&1& no clouds, elongation due to refraction ~1.4 airmass. 6780 lost\\
ML02&130613&09:14&.65&1& redo wavefront and switch to r filter\\
ML02&130613&09:30&.7&1& \\
ML02&130613&09:42&.8&1& \\
ML02&130613&09:55&.9&1& getting to high airmass\\
MM01&130702&03:41&0.50-0.55${^\prime^\prime}$&1& 15x120 \\
MM02&130702&04:26&0.60-0.70${^\prime^\prime}$&1& 15x120  \\
MM01&130702&05:10&0.60-0.70${^\prime^\prime}$&1& 12x120\\
MM02&130702&05:42&0.55-0.80${^\prime^\prime}$&1& 12x120\\
MM01&130702&06:17&0.50-0.90${^\prime^\prime}$&1& 12x120 \\
MM02&130702&06:52&0.55-0.65${^\prime^\prime}$&1& 12x120\\
MM01&130703&03:50&0.60-0.80${^\prime^\prime}$&1& 12x120\\
MM02&130703&04:22&0.60-0.80${^\prime^\prime}$&1& 12x120\\
MM01&130703&04:56&0.55-0.60${^\prime^\prime}$&1& 12x120\\
MM02&130703&06:13&0.55-0.65${^\prime^\prime}$&1& 12x120\\
MM01&130703&06:48&0.60-0.65${^\prime^\prime}$&1& 12x120 some elongation\\
MM02&130703&07:23&0.70-1.00${^\prime^\prime}$&1& 6x120 \\
MM01&130704&03:40&0.70-0.90${^\prime^\prime}$&1& 6x120\\
MM01&130704&04:27&0.60-0.75${^\prime^\prime}$&1& 12x120\\
MM01&130704&05:07&0.75-0.90${^\prime^\prime}$&1& 12x120\\
MM01&130704&06:09&1.00-1.20${^\prime^\prime}$&1& 12x120\\
MM01&130704&06:42&1.00-1.20${^\prime^\prime}$&1& 6x120 \\
MM03&130707&05:42&1.10-1.20${^\prime^\prime}$&1& 12x120\\
MM03&130707&06:20&1.00-1.10${^\prime^\prime}$&1& 12x120\\
MM03&130707&06:56&0.90-1.10${^\prime^\prime}$&1& 12x120\\
SM01&130704&07:15&1.2&1& .\\
SM02&130704&08:15&1.3&1& .\\
SM01&130704&09:16&1.2&1& .\\
SM02&130704&10:16&1.1&1& .\\
SM01&130704&11:23&1.2&1& .\\
SM02&130704&12:22&1.3&1& .\\
SM01&130705&07:08&1.7&1& .\\
SM02&130705&08:07&1.2&1& .\\
SM01&130705&09:14&0.9&1& .\\
SM02&130705&10:14&0.9&1& .\\
SM01&130705&11:13&0.9&1& .\\
SM02&130705&12:13&0.9&1& .\\
SM01&130706&07:03&0.6&1& .\\
SM02&130706&08:03&0.6&1& .\\
SM01&130706&09:10&0.7&1& .\\
SM02&130706&10:10&0.7&1& .\\
SM01&130706&11:10&0.8&1& .\\
SM02&130706&12:10&0.7&1& .\\
SM03&130707&07:01&0.9&2& some cirrus around\\
SM04&130707&08:01&0.8&1& .\\
SM03&130707&09:01&0.9&1& .\\
SM04&130707&10:01&0.9&2& some cirrus\\
SM03&130707&11:01&0.9&1& focus went off but got it back\\
SM04&130707&12:01&0.7&1& .\\
SM03&130710&06:58&1.7&1& . \\
SM04&130710&07:57&1.3&1& .\\
SM03&130710&08:57&1.4&1& .\\
SM04&130710&09:57&1.4&1& .\\
SM03&130710&10:57&2.3&1& .\\
SM04&130710&11:57&1.9&1& .\\
SM03&130714&07:00&0.67&1& Fairly clear.  Approx log made from  notes\\
SM04&130714&08:00&0.67&1& Fairly clear.  Approx log made from  notes\\
SM03&130714&09:00&0.67&2& Thin cirrus.  Approx log made from notes\\
SM04&130714&10:00&0.67&2& Thin cirrus.  Approx log made from notes\\
SM03&130714&11:00&0.67&2& Thin cirrus.  Approx log made from notes\\
MN01&130828&00:30&0.80${^\prime^\prime}$&1& 10 and 30s gr astrometric frames\\
MN01&130828&00:32&0.60-0.75${^\prime^\prime}$&1& 15x120 gr\\
MN01&130828&01:16&0.70-0.80${^\prime^\prime}$&1& 15x120 gr\\
MN01&130828&01:55&0.75-0.85${^\prime^\prime}$&1& 12x120 gr\\
MN01&130828&02:34&0.75-0.85${^\prime^\prime}$&1& 9x120 gr elongated\\
MN01&130828&02:58&0.65-0.90${^\prime^\prime}$&1& 11x120 try r filter for comparison set, \& check on elongation \\
MN01&130828&03:35&0.75-0.80${^\prime^\prime}$&1& 4x120 r\\
MN01&130828&23:27&0.45-0.55${^\prime^\prime}$&1& 15x120 gr\\
MN01&130829&00:16&0.40-0.50${^\prime^\prime}$&1& 20x120 gr\\
MN01&130829&01:10&0.35-0.45${^\prime^\prime}$&1& 18x120 gr\\
MN01&130829&02:01&0.50-0.60${^\prime^\prime}$&1& 15x120 gr\\
MN01&130829&02:43&0.50-0.60${^\prime^\prime}$&1& 15x120 gr some elongation coming in  \\
MN01&130829&03:21&0.60-0.70${^\prime^\prime}$&1& 15x120 gr some elongation from refraction\\
MN01&130829&23:47&0.70-0.80${^\prime^\prime}$&1& 3x120 gr\\
MN01&130829&23:54&0.60-0.65${^\prime^\prime}$&1& 11x120 gr\\
MN01&130830&00:27&0.65-0.70${^\prime^\prime}$&1& 7x120 gr some horizontal elongation\\
MN01&130830&00:45&0.60-0.65${^\prime^\prime}$&1& 11x120 gr\\
MN01&130830&01:17&0.70-0.80${^\prime^\prime}$&1& 15x120 gr\\
MN01&130830&01:55&0.70-0.80${^\prime^\prime}$&1& 15x120 gr\\
MN01&130830&02:42&0.75-0.85${^\prime^\prime}$&1& 15x120 gr\\
MN01&130830&03:28&0.85-1.00${^\prime^\prime}$&1& 9x120 gr elongation from refraction\\
MN01&130831&23:25&0.75${^\prime^\prime}$&1& 10s and 30s gr astrometric frames 3x120s gr \\
MN01&130831&23:42&0.70-0.90${^\prime^\prime}$&1& 15x120 gr\\
MN01&130901&00:24&0.75-0.85${^\prime^\prime}$&1& 15x120 gr\\
MN01&130901&01:09&0.70-0.80${^\prime^\prime}$&1& 15x120 gr\\
MN01&130901&01:49&0.65-0.80${^\prime^\prime}$&1& 15x120 gr\\
MN01&130901&02:32&0.80-0.90${^\prime^\prime}$&1& 7x120 gr\\
MN01&130901&03:06&0.75-0.90${^\prime^\prime}$&2& 15x120 gr some cloud intermittent\\
MN01&130902&23:34&0.65-0.75${^\prime^\prime}$&1& 15x120 gr\\
MN01&130903&00:18&0.55-0.75${^\prime^\prime}$&1& 15x120 gr\\
MN01&130903&01:01&0.60-0.70${^\prime^\prime}$&1& 15x120 gr one frame at 0.8 tracking seeing variations\\
MN01&130903&01:45&0.85-1.00${^\prime^\prime}$&1& 15x120 gr\\
MN01&130903&02:32&0.75-0.80${^\prime^\prime}$&1& 8x120 gr\\
MN01&130904&23:43&0.55-0.65${^\prime^\prime}$&2& 15x120 gr not photometric 1-10\%\\
MN01&130904&00:39&0.50-0.65${^\prime^\prime}$&2& 20x120 gr not photometric 1-50\%\\
MN01&130904&01:37&0.55-0.60${^\prime^\prime}$&2& 15x120 gr not photometric 1-50\%\\
MN01&130904&02:21&0.50-0.60${^\prime^\prime}$&2& 8x120 gr not photometric 10-50\%\\
MN01&130906&23:25&0.50-0.60${^\prime^\prime}$&1& 15x120 gr  cirrus but clear at pointing\\
MN01&130906&00:09&0.45-0.50${^\prime^\prime}$&1& 20x120 gr  cirrus but clear at pointing\\
MN01&130906&00:51&0.45-0.55${^\prime^\prime}$&1& 7x120 gr  cirrus but clear at pointing\\
MN01&130906&01:09&0.50-0.60${^\prime^\prime}$&2& 8x120 gr not photometric  cirrus passing\\
MN01&130906&01:32&0.50-0.65${^\prime^\prime}$&2& 15x120 gr not photometric  cirrus 1-70\%\\
MN01&130906&02:16&0.55-0.65${^\prime^\prime}$&2& 15x120 gr not photometric  cirrus 1-50\%\\
MN01&130906&02:59&0.60-0.65${^\prime^\prime}$&2& 6x120 gr not photometric  cirrus 10-50\%\\
MO01&140425&05:57&0.60${^\prime^\prime}$&1& 20x120 gr elongated from filter at airmass \\
MO01&140425&06:53&0.50-0.55${^\prime^\prime}$&1& 20x120 gr\\
MO01&140425&07:48&0.45-0.50${^\prime^\prime}$&1& 15x120 gr\\
MO01&140425&08:26&0.55-0.60${^\prime^\prime}$&1& 7x120 gr some wind shake, elongation\\
MO01&140425&08:49&0.40-0.50${^\prime^\prime}$&1& 20x120 gr \\
MO01&140425&09:48&0.50-0.60${^\prime^\prime}$&1& astrometric frames 10s and 30s\\
MO02&140425&09:52&0.50-0.60${^\prime^\prime}$&1& astrometric frames 10s and 30s\\
MO02&140425&09:54&0.55-0.60${^\prime^\prime}$&1& 3x120 gr test frames with bkg increasing \\
MO03&140425&10:07&0.50-0.60${^\prime^\prime}$&1& astrometric frames 10s and 30s\\
MO01&140426&09:01&0.65-1.0${^\prime^\prime}$&2& 24x120 gr only 4 frames at 0.65${^\prime^\prime}$\\
MO01&140427&08:19&0.55-0.75${^\prime^\prime}$&1& 6x120 gr \\
MO01&140427&08:34&0.55-0.75${^\prime^\prime}$&2& 10x120 gr clouds progressively more extinction\\
MO01&140428&07:43&0.50-0.60${^\prime^\prime}$&1& 20x120 gr \\
MO01&140428&08:40&0.50-0.60${^\prime^\prime}$&1& 20x120 gr \\
MO01&140428&09:31&0.50-0.65${^\prime^\prime}$&1& 14x120 gr last 4 frames have rising bkg levels \\
MO02&140429&07:09&0.55-0.70${^\prime^\prime}$&1& 20x120 gr some wind shake  \\
MO02&140429&08:04&0.60-0.75${^\prime^\prime}$&1& 20x120 gr some wind shake \\
MO02&140429&07:09&0.65-0.80${^\prime^\prime}$&2& 20x120 gr thin cloud spreading about half\\
MO02&140430&07:07&0.40-0.50${^\prime^\prime}$&1& 20x120 gr \\
MO01&140430&08:05&0.40-0.50${^\prime^\prime}$&1& 20x120 gr \\
MO02&140430&08:58&0.40-0.50${^\prime^\prime}$&1& 20x120 gr \\
MO02&140430&08:58&0.50-0.50${^\prime^\prime}$&2& 10x120 gr bkg increasing in last 5 frames\\
MO02&140501&08:56&0.65-0.90${^\prime^\prime}$&3& 20x120 gr clouds variable extinction 0.2-1.0 mag\\
MO02&140502&07:06&0.55-0.75${^\prime^\prime}$&1& 20x120 gr \\
MO03&140502&08:05&0.50-0.65${^\prime^\prime}$&1& 20x120 gr \\
MO02&140502&09:03&0.55-0.60${^\prime^\prime}$&1& 20x120 gr \\
MO02&140502&09:58&0.60-0.65${^\prime^\prime}$&2& 5x120 gr bkg increasing\\
MO03&140504&08:22&0.55-0.65${^\prime^\prime}$&1& 17x120 gr \\
MO03&140504&09:17&0.45-0.60${^\prime^\prime}$&1& 15x120 gr \\
MO03&140504&09:54&0.60-0.70${^\prime^\prime}$&2& 4x120 gr bkg increasing\\
MO03&140505&06:22&0.70-0.90${^\prime^\prime}$&1& 20x120 gr \\
MO03&140505&07:17&0.76-0.95${^\prime^\prime}$&1& 20x120 gr \\
MO02&140505&08:12&0.80-1.10${^\prime^\prime}$&1& 15x120 gr \\
MO03&140505&09:35&0.75-1.00${^\prime^\prime}$&1& 13x120 gr  bkg increasing on last 3 frames\\
MO03&140506&05:54&0.40-0.45${^\prime^\prime}$&1& 20x120 gr \\
MO02&140506&06:49&0.35-0.43${^\prime^\prime}$&1& 20x120 gr \\
MO03&140506&07:44&0.45-0.55${^\prime^\prime}$&2& 20x120 gr thin cloud crossing 0.1-0.25 mag ext\\
MO03&140506&08:35&0.40-0.50${^\prime^\prime}$&1& 20x120 gr maybe some very thin cloud still passing\\
MO01&140506&09:27&0.42-0.55${^\prime^\prime}$&1& 15x120 gr \\
MO01&140506&10:04&0.60${^\prime^\prime}$&1& 1x120 gr bkg coming up\\
Deep05&140625&07:55&0.7${^\prime^\prime}$&4& 30s off galaxy image, HSCA00296800.fits\\
SP01&140625&08:00&0.80${^\prime^\prime}$&4& 30s in galaxy on SP01, HSCA00297200.fits\\
SP01&140625&08:05&0.80${^\prime^\prime}$&1& 90s HSCA00297400.fits \\
SP01&140625&08:30&0.60${^\prime^\prime}$&1& 90s HSCA00300200.fits\\
SP01&140625&09:00&0.62${^\prime^\prime}$&1& 90s HSCA00302200.fits\\
SP01&140625&09:30&0.53${^\prime^\prime}$&1& 90s HSCA00304600.fits\\
SP01&140625&10:00&0.48${^\prime^\prime}$&1& 90s HSCA00308200.fits\\
SP01&140625&10:30&0.55${^\prime^\prime}$&1& 90s HSCA00311000.fits\\
SP01&140625&11:00&0.58${^\prime^\prime}$&1& 90s HSCA00313600.fits\\
SP01&140625&11:30&0.54${^\prime^\prime}$&1& 90s HSCA00316800.fits\\
SP01&140625&12:10&0.53${^\prime^\prime}$&1& 90s HSCA00319200.fits\\
SP01&140625&13:00&0.57${^\prime^\prime}$&1& 90s HSCA00324200.fits\\
SP01&140625&13:22&0.58${^\prime^\prime}$&1& 90s HSCA00326000.fits\\
SP01&140625&13:35&0.63${^\prime^\prime}$&1& 90s HSCA00327200.fits\\
SP01&140625&13:40&0.69${^\prime^\prime}$&1& 90s HSCA00327600.fits\\
SP01&140627&08:05&0.48${^\prime^\prime}$&1& 90s HSCA00335800.fits\\
SP01&140627&08:35&0.52${^\prime^\prime}$&1& 90s HSCA00338000.fits\\
SP01&140627&09:10&0.49${^\prime^\prime}$&1& 90s HSCA00340800.fits\\
SP01&140627&09:28&0.55${^\prime^\prime}$&1& 90s HSCA00343000.fits\\
SQ01&140726&06:05&0.60&1&   0.55 - 0.65${^\prime^\prime}$  10 frames, 147294-147303\\
SQ01&140726&06:25&0.60&1&   0.55 - 0.65${^\prime^\prime}$  11 frames, 147304-147314\\
SQ01&140726&06:47&0.52&1&   0.49 - 0.55${^\prime^\prime}$  10 frames, 147315-147324\\
SQ03&140726&07:25&0.53&1&   0.48 - 0.57${^\prime^\prime}$  10 frames, 147328-147337\\
SQ03&140726&07:45&0.60&1&   0.50 - 0.72${^\prime^\prime}$  10 frames, 147338-147347\\
SQ03&140726&08:05&0.60&1&   0.57 - 0.67${^\prime^\prime}$  10 frames, 147348-147357\\
SQ01&140726&08:34&0.60&1&   0.51 - 0.67${^\prime^\prime}$  10 frames, 147359-147368\\
SQ01&140726&08:53&0.56&1&   0.53 - 0.60${^\prime^\prime}$  10 frames, 147369-147378\\
SQ01&140726&09:15&0.52&1&   0.50 - 0.53${^\prime^\prime}$  10 frames, 147379-147388\\
SQ03&140726&09:34&0.55&1&   0.49 - 0.61${^\prime^\prime}$  10 frames, 147389-147398\\
SQ03&140726&09:54&0.67&1&   0.67 - 0.69${^\prime^\prime}$  10 frames, 147399-147408\\
SQ03&140726&10:14&0.80&1&   0.77 - 0.85${^\prime^\prime}$  10 frames, 147409-147418\\
SQ02&140726&10:40&0.80&1&   0.70 - 0.87${^\prime^\prime}$  10 frames, 147421-147430\\
SQ02&140726&11:01&0.80&1&   0.74 - 0.88${^\prime^\prime}$  10 frames, 147431-147440\\
SQ02&140726&11:21&0.80&1&   0.74 - 0.85${^\prime^\prime}$  10 frames, 147441-147450\\
SQ02&140727&06:05&0.90&1&   0.82 - 1.07${^\prime^\prime}$  10 frames, 147537-147546\\
SQ02&140727&06:25&0.95&1&   0.82 - 1.07${^\prime^\prime}$  13 frames, 147547-147559\\
SQ02&140727&07:09&0.68&1&   0.61 - 0.76${^\prime^\prime}$  10 frames, 147561-147570\\
SQ02&140727&07:29&0.66&1&   0.65 - 0.68${^\prime^\prime}$  10 frames, 147571-147580\\
SQ02&140727&07:49&0.82&1&   0.77 - 0.90${^\prime^\prime}$  10 frames, 147581-147590\\
SQ03&140727&08:09&0.78&1&   0.74 - 0.82${^\prime^\prime}$  10 frames, 147591-147600\\
SQ03&140727&08:29&0.71&1&   0.72 - 0.73${^\prime^\prime}$  10 frames, 147601-147610\\
SQ03&140727&08:49&0.71&1&   0.67 - 0.77${^\prime^\prime}$  10 frames, 147611-147620\\
SQ01&140727&09:17&0.74&1&   0.68 - 0.77${^\prime^\prime}$  10 frames, 147622-147631\\
SQ01&140727&09:37&0.73&1&   0.68 - 0.81${^\prime^\prime}$  10 frames, 147632-147641\\
SQ01&140727&09:57&0.78&1&   0.70 - 0.82${^\prime^\prime}$  10 frames, 147642-147651\\
SQ02&140727&10:18&0.84&1&   0.82 - 0.88${^\prime^\prime}$  10 frames, 147652-147661\\
SQ02&140727&10:38&0.84&1&   0.83 - 0.85${^\prime^\prime}$  10 frames, 147662-147671\\
SQ02&140727&10:58&0.91&1&   0.88 - 0.95${^\prime^\prime}$  10 frames, 147672-147681\\
SQ02&140727&11:18&0.88&1&   0.79 - 0.93${^\prime^\prime}$  9 frames, 147682-147690\\
\enddata
\end{deluxetable}



==> tbl11obj.tex <==
% This started from Susan's table, MarcTables.docx

\startlongtable
\begin{deluxetable}{chhccccccccccccc}
\tabletypesize{\scriptsize}
\tablecaption{Summary of 2011-2013 Search Discoveries\label{tbl-11obj}}
\tablewidth{0pt}
\tablehead{
\colhead{Object}&
\nocolhead{AHP-ID}&
\nocolhead{MWB-ID}&
\colhead{$a$}&
\colhead{$e$}&
\colhead{$i$}&
\colhead{$H_V$}&
\colhead{$R$}&
\colhead{arc}&
\colhead{discovery}&
\colhead{Nobs}&
\colhead{Desig}&
\colhead{type}&
\colhead{CA Date}&
\colhead{CA}&
\colhead{$\Delta$V}\\
&
&
&
(AU)&
&
(deg)&
&
&
(days)&
(UT)&
&
&
&
(UT)&
(AU)&
m/sec
}
\startdata
VNH0008& MA01c15a& NI112& 44.00$\pm$0.01&  0.04&   2.60&     8.6&    24.5&  358& 2011-04-28&  36& 2011JY31&        C& 2018-10-07&    0.15&     245\\
VNH0010& MA04c28a& NI113& 43.15$\pm$0.03&  0.03&   2.39&     9.4&    25.4&  359& 2011-04-28&  33& 2011HZ102&       C& 2018-11-09&    0.16&     250\\
VNH0007& MA01c12a& NI124&    46$\pm$1&     0.14&   1.87&     9.3&    25.2&  357& 2011-04-29&  20& 2011JW31&        C& 2018-08-22&    0.16&     259\\
VNH0006& MA04c06a& NI115&    51$\pm$26&    0.02&   2.51&     9.2&    26.0&    3& 2011-04-30&   6& \nodata&   \nodata& 2021-07-01&    0.38&     318\\
VNH0009& MA04c14d& NI104&  45.2$\pm$0.6&   0.13&   3.31&     8.2&    24.5&  359& 2011-04-28&  54& 2011JX31&        C& 2020-07-15&    0.36&     358\\
VNH0050&         & NI194&    45$\pm$23&    0.02&   2.90&    11.6&    27.7& 0.08& 2013-06-07&   3& \nodata&   \nodata& 2019-05-21&    0.3&      375\\
VNH0036& ML02c12a& NI199&    43$\pm$22&    0.03&   1.88&    12.2&    28.2&    3& 2013-06-04&   9& \nodata&   \nodata& 2018-09-18&    0.26&     421\\
VNH0044&         & NI187&    48$\pm$21&    0.33&   3.40&    13.0&    29.2&   33& 2013-06-03&  14& \nodata&   \nodata& 2020-09-25&    0.45&     435\\
VNH0002& MC07c02a& NI111& 53.34$\pm$0.05&  0.31&   6.42&    11.3&    27.3&  862& 2011-04-28&  55& 2011HK103&       S& 2019-09-01&    0.27&     441\\
VNH0005& MC06c03a& NI105&  43.0$\pm$0.2&   0.04&   3.05&    11.0&    27.0&  446& 2011-04-29&  24& 2011HF103&       C& 2018-12-12&    0.30&     445\\
VNH0034& ML03c03a& NI180&    44$\pm$1&     0.06&   2.99&    12.3&    28.4&   94& 2013-06-05&  18& 2013LU35&        C& 2019-04-20&    0.33&     450\\
VNH0029&         & NI156&    67$\pm$31&    0.04&   2.77&     9.7&    27.7&    5& 2011-04-28&   5& \nodata&   \nodata& 2027-06-01&    1.1&      457\\
VNH0054&         & NI179&    47$\pm$47&    0.03&   2.65&    13.0&    29.4&    1& 2012-04-17&   6& \nodata&   \nodata& 2019-11-16&    0.42&     492\\
VNH0019& MF01c02a&      &    46$\pm$10&    0.02&   2.68&     8.3&    24.7&    2& 2012-04-17&   6& \nodata&   \nodata& 2019-12-24&    0.44&     505\\
VNH0052&         & NI196&    44$\pm$23&    0.25&   2.57&    13.1&    29.1&    5& 2013-06-06&   7& \nodata&   \nodata& 2019-06-07&    0.43&     562\\
VNH0021& MF01c16a& NI174& 44.42$\pm$0.03&  0.10&   3.03&    12.8&    28.5&  506& 2012-04-18&  42& \nodata&       9:5& 2017-12-09&    0.32&     716\\
VNH0014& MA04c21c& NI163&    56$\pm$17&    0.44&   3.22&    12.2&    28.3&  355& 2011-05-02&  19& 2011JA32&        C& 2018-02-10&    0.38&     767\\
VNH0058&         & NI190&    42$\pm$22&    0.02&   2.19&    12.4&    28.1&    7& 2013-07-07&   6& \nodata&   \nodata& 2018-04-20&    0.41&     771\\
VNH0017&         &      &    47$\pm$24&    0.26&   6.72& \nodata& \nodata&   33& 2011-04-28&  10& \nodata&   \nodata& 2021-02-02&    0.93&     833\\
VNH0040&         & NI169&    48$\pm$25&    0.02&   3.17&    11.7&    28.1&    1& 2011-07-23&   3& \nodata&   \nodata& 2020-05-05&    0.85&     886\\
VNH0003& MC07c02b& NI107&    47$\pm$2&     0.19&   5.36&    10.8&    26.5&   65& 2011-04-28&  22& 2011HJ103&       C& 2017-10-13&    0.40&     949\\
VNH0012& MA01c25a& NI162&  43.7$\pm$0.2&   0.08&   6.83&    12.6&    29.1&  357& 2011-04-28&  24& 2011HE103& \nodata& 2020-04-18&    0.92&     975\\
VNH0022& MF01c23a& NI177&  46.2$\pm$0.4&   0.21&   5.44&    13.1&    29.0&  505& 2012-04-17&  35& 516977&          S& 2017-12-10&    0.49&    1.1k\\
VNH0033& ML01c31a& NI193&    58$\pm$30&    0.58&   5.93&    10.5&    27.7&   10& 2013-06-03&  16& \nodata&   \nodata& 2022-05-10&    1.5&     1.1k\\
VNH0025&         & NI101&    46$\pm$24&    0.02&   2.92&     8.6&    24.9&    1& 2011-05-31&   5& \nodata&   \nodata& 2019-09-25&    1.0&     1.2k\\
VNH0016& MA04c35a& NI114&    53$\pm$27&    0.49&   5.76&    11.2&    28.1&  358& 2011-04-28&  24& 2011HD103& \nodata& 2020-11-11&    1.4&     1.3k\\
VNH0047& ML02c03b&      &    47$\pm$24&    0.02&  14.55&    11.1&    28.1& 0.12& 2013-06-06&   3& \nodata&   \nodata& 2020-01-10&    1.4&     1.5k\\
VNH0046&         & NI189&    45$\pm$23&    0.02&   7.43&    12.1&    28.1& 0.17& 2013-07-07&   3& \nodata&   \nodata& 2019-05-22&    1.2&     1.6k\\
VNH0027& ML01c14a& NI110&    54$\pm$29&    0.76&   6.95&    10.4&    27.0&  703& 2011-07-02&   8& \nodata&   \nodata& 2023-05-11&    2.5&     1.6k\\
VNH0037&         &      &    58$\pm$30&    0.02&  13.83&    10.6&    27.8& 0.08& 2011-07-01&   2& \nodata&   \nodata& 2023-10-23&    2.7&     1.6k\\
VNH0035& ML01c23a&      &    42$\pm$22&    0.02&  12.75&     9.1&    24.8&    2& 2013-06-11&   4& \nodata&   \nodata& 2018-03-05&    0.84&    1.7k\\
VNH0055&         & NI182&    48$\pm$18&    0.23&   6.96&    13.3&    28.9&   33& 2013-06-03&  14& \nodata&   \nodata& 2018-03-17&    0.86&    1.7k\\
VNH0032& ML01c08a&      &    41$\pm$21&    0.02&   7.62&    10.2&    25.9&    4& 2013-06-04&   6& \nodata&   \nodata& 2018-01-28&    0.90&    1.9k\\
VNH0020& MF01c08a& NI178&    58$\pm$28&    0.24&  10.20&    12.8&    29.0&    1& 2012-04-18&  15& \nodata&   \nodata& 2019-03-30&    1.4&     2.0k\\
VNH0026&         & NI109&    45$\pm$23&    0.02&   9.08&     8.9&    25.0& 0.19& 2011-07-02&   3& \nodata&   \nodata& 2019-04-19&    1.7&     2.3k\\
VNH0061& ML02c03a&      &    45$\pm$23&    0.02&  16.06&     9.7&    25.8& 0.12& 2013-06-05&   3& \nodata&   \nodata& 2019-04-26&    1.8&     2.4k\\
VNH0059&         & NI192&    87$\pm$3&     0.57&   9.91&    12.4&    28.0&   88& 2013-06-08&  19& \nodata&         S& 2017-09-29&    1.1&     2.8k\\
VNH0051&         & NI195&    43$\pm$18&    0.06&  12.01&    12.6&    28.5&    6& 2013-06-05&   9& \nodata&   \nodata& 2018-06-28&    1.6&     2.8k\\
VNH0024& MF01c31a& NI175&  41.7$\pm$0.9&   0.15&   4.56&    12.2&    27.4&    3& 2012-04-17&  23& \nodata&   \nodata& 2016-05-01&    0.34&    3.0k\\
VNH0018&         &      &    45$\pm$23&    0.02&  16.61& \nodata& \nodata& 0.06& 2011-06-01&   8& \nodata&   \nodata& 2019-04-01&    2.3&     3.2k\\
VNH0060&         & NI198&    40$\pm$12&    0.09&   7.26&    13.3&    28.8&    8& 2013-06-05&   9& \nodata&   \nodata& 2017-03-29&    1.0&     3.4k\\
VNH0042&         & NI183&    40$\pm$20&    0.03&  19.92&    12.7&    28.4&    2& 2013-07-04&   4& \nodata&   \nodata& 2018-01-29&    1.9&     4.0k\\
VNH0045&         & NI188&    39$\pm$20&    0.02&  18.89&    13.4&    28.8&    7& 2013-07-07&   6& \nodata&   \nodata& 2017-03-15&    1.6&     5.3k\\
VNH0023& MF01c26a& NI176&    39$\pm$3&     0.02&  19.28&    12.8&    28.4&    2& 2012-04-17&  18& \nodata&   \nodata& 2017-03-29&    1.6&     5.3k\\
VNH0057&         & NI186&    41$\pm$22&    0.02&  31.74&    12.4&    28.1&    1& 2013-07-05&   5& \nodata&   \nodata& 2018-01-03&    2.5&     5.4k\\
VNH0011& MA01c17a& NI100&  42.3$\pm$0.8&   0.15&  14.44&     7.9&    25.4&   65& 2011-04-28&  25& 2011HL103&     5:3& 2016-08-29&    1.4&     7.8k\\
VNH0041& MM01c26a& NI181&    45$\pm$19&    0.62&  12.20&    11.9&    27.3&   23& 2013-06-13&  15& \nodata&   \nodata& 2016-07-11&    1.3&     8.3k\\
VNH0013& MA04c16a& NI103&    54$\pm$8&     0.41&  12.94&    11.5&    26.7&   63& 2011-04-30&  39& 2011JD32&  \nodata& 2015-12-26&    1.1&    25.9k\\
VNH0001& MC04c01b& NI108& 30.12$\pm$0.01&  0.08&  29.38&     8.6&    22.8&  354& 2011-04-29& 131& 2011HM102&     1:1& 2013-11-04&    1.2&  \nodata\\
VNH0031&         & NI164&    23$\pm$23&    0.32&   6.94&    14.1&    28.6&    5& 2011-04-28&   5& \nodata&   \nodata& 2014-06-29&    0.73& \nodata\\
VNH0048&         & NI191&    37$\pm$9&     0.25&  22.34&    14.1&    28.5&    9& 2013-06-04&  12& \nodata&   \nodata& 2014-07-02&    1.3&  \nodata\\
VNH0004& MC02c05a& NI102&    37$\pm$14&    0.30&   3.81&    10.8&    25.6&   34& 2011-05-29&  12& 2011KW48&  \nodata& 2015-02-12&    0.43& \nodata\\
VNH0053&         & NI197&    34$\pm$18&    0.25&  25.09&    13.7&    28.4&    4& 2013-06-09&   9& \nodata&   \nodata& 2015-06-12&    0.95& \nodata\\
VNH0056&         & NI184&    42$\pm$21&    0.61&  16.00&    13.0&    28.0&   23& 2013-06-13&   9& \nodata&   \nodata& 2015-10-15&    0.90& \nodata\\
VNH0015& MA04c34a&      &    35$\pm$21&    0.03&  18.95&    10.4&    25.5&    5& 2011-04-28&   6& \nodata&   \nodata& 2015-10-21&    1.8&      $>$\\
VNH0039&         &      &  2000$\pm$1200&  0.84& 171.95& \nodata&    26.8& 0.11& 2011-07-02&   2& \nodata&   \nodata&    \nodata& \nodata& \nodata\\
\enddata
\tablecomments{\scriptsize
$R$ magnitude is the apparent brightness at the time of discovery
}
\end{deluxetable}

